Regularization for Design

When designing controllers for large-scale systems, the architectural aspects of the controller such as the placement of actuators, sensors, and the communication links between them can no longer be taken as given. The task of designing this architecture is now as important as the design of the control laws themselves. By interpreting controller synthesis (in a model matching setup) as the solution of a particular linear inverse problem, we view the challenge of obtaining a controller with a desired architecture as one of finding a structured solution to an inverse problem. Building on this conceptual connection, we formulate and analyze a framework called \textit{Regularization for Design (RFD)}, in which we augment the variational formulations of controller synthesis problems with convex penalty functions that induce a desired controller architecture. The resulting regularized formulations are convex optimization problems that can be solved efficiently, these convex programs provide a unified computationally tractable approach for the simultaneous co-design of a structured optimal controller and the actuation, sensing and communication architecture required to implement it. Further, these problems are natural control-theoretic analogs of prominent approaches such as the Lasso, the Group Lasso, the Elastic Net, and others that are employed in statistical modeling. In analogy to that literature, we show that our approach identifies optimally structured controllers under a suitable condition on a "signal-to-noise" type ratio.

==> app_lem3.tex <==
\begin{lem}
Suppose that $t$ and $v$ are chosen such that Assumption \ref{as:nu} holds, and $\lambda = \lambda^{\leq t,v} + \kappa$, where $\lambda^{\leq t,v}$ is given by the right hand side of \eqref{eq:sufficient}, and $\kappa>0$ is an arbitrarily small constant.  Further, let the noise term $\Noise$ be as in \eqref{eq:noise}. Then if $\gtv > \btv$, all components $(U^{\leq v}_*)_\Aa$ such that
\begin{equation}
\begin{array}{l}
\left(\Gdnorm{{U^{\leq v}_*}} - \Htwonorm{{(U^{\leq v}_*)_\Aa}}\right) <  \frac{\left(\gtv-\btv\right)\Gdnorm{{U^{\leq v}_*}} - \Noise}{\rho + \gtv - \btv}
\end{array}
\label{eq:gap}
\end{equation}
satisfy condition \eqref{eq:structure} for sufficiently small $\kappa$.
\label{lem:rho_lemma}
\end{lem}
\begin{IEEEproof}
Relation \eqref{eq:gap} follows from rearranging terms in \eqref{eq:structure}, and then letting $\kappa$ tend to 0 from above.
\end{IEEEproof}

==> case_studies.tex <==
%The definition of the SNR \eqref{eq:groupSNR} has clear implications on the types of controllers that are easily recovered by the RFD optimization problem \eqref{eq:Topt} \todo{check reference}.  \todo{make active, rather than passive}.  In particular, controllers with large initial impulse response elements (i.e. with large $\Htwonorm{(U^{\leq v}_*)_\Aa}$) and small tail effects (i.e. with small $\drv$) that achieve a small closed loop norm (i.e. those with small $W^{\leq t}$).  Further controllers with more evenly spread out actuation (i.e. that maximize $\tau_{\Gs}$) enjoy a large $\gtv$ for a broader range of $t$.  \todo{punchline linking to the threshold condition -- need LHS big, and RHS small.  We get LHS big if (a), and RHS small if (b)}.
%
%\todo{in particular if we have "sparse controllers" (dispersed actuation) that achieve a good closed loop performance (i.e. act quickly and aggressively) will enjoy these characteristics and satisfy our sufficient conditions.}
%Sparse controllers achieving good closed loop performance are likely to have these characteristics.  In particular, since actuation is sparse, much of the system is essentially operating in open-loop -- as such, actuators that are present should be approximately evenly dispersed, and should act quickly and aggressively to suppress local disturbances.

The following case study illustrates the concepts introduced in the previous section on a concrete system that satisfies our sufficient conditions.

\begin{figure}[h!]
\centering
\includegraphics[width = .35\textwidth]{chain}
\caption{A diagram of the Stable Unidirectional Chain System case study.}
\label{fig:chain}
\end{figure}

We consider a $\Htwo$ RFD optimization with control cost $\rho_u = .1$, and the remaining generalized plant \eqref{eq:genplant} state space parameters set as $B_2=C_1=I_{10}$, $A = \frac{1}{2}I_{10} + \frac{1}{2}Z_{10}$, and \edit{$B_1 = 1.1(E_{11} + E_{55}) + .7 E_{99} + .1 I_{10}$}.  This system is illustrated in Figure \ref{fig:chain}.  
This simple example is chosen in order to allow a direct computation of various bounds and parameters, and to easily interpret the propagation of inputs and disturbances.

We consider the task of recovering the optimal actuation schemes that use either 2 actuators or 3 actuators.    In particular, we take the desired controller $U_s$, for $s=2$ and $s=3$, to be 
\begin{equation}
\begin{array}{rl}
U_s := \argmin{U \in \RHinf}&\Htwonorm{Y-\M(U)}^2 + .1\Htwonorm{U}^2 \\
\text{s.t.} & \text{\edit{$U$ has at most $s$ nonzero rows}},
\end{array}
\label{eq:chainUs}
\end{equation}
with open loop state response $Y$ and map from the Youla parameter to state component of the closed loop response $\M$ as defined in Example \ref{ex:actuators}.  We solve this optimization problem by enumerating all possible actuation schemes, and we find that the optimal actuation scheme for $s=2$ is given by actuators at nodes $1$ and $5$, and for $s=3$ by actuators at nodes $1$, $5$ and $9$.

\edit{We emphasize that the goal of this case study is to illustrate the concepts introduced in the previous section, and to help the reader understand how the various parameters affect the recovery conditions -- in practice, $\m_*$ and $\Aa_*$ are not available.  Further, we note that the case study presented is the first example in the literature of a system for which convex optimization provably identifies an optimal actuation architecture}

With these optimal actuation schemes at our disposal, we vary the parameters $t$ and $v$ to investigate how our recovery conditions are affected -- \edit{in practice, a suitable horizon $t$ and controller order $v$ would be chosen empirically}.  As per the discussion in $\S\ref{sec:parameters}$, we set $\rho=0$.  We also show that for appropriate fixed controller order $v$ and horizon $t$, increasing $\lambda$ shifts the identified architecture from actuators at nodes 1, 5 and 9 to actuators at nodes 1 and 5.  This is a very desirable property form an architecture design perspective, as it suggests that increasing the regularization weight $\lambda$ causes the identified architecture to move to a simpler, but still optimal, actuator configuration.  \edit{In practice, $\lambda$ would be chosen empirically, but as predicted by Corollary \ref{coro:success}, each optimal architecture is identified for a range of regularization weights $\lambda$.  Further, as predicted by Theorem \ref{thm:main}, the identified architectures are those for which the optimal control law achieves a small closed loop state response.}


%\todo{General discussion: identify optimally structured actuation schemes with 2 actuators and 3 actuators by solving the following problem (via combinatorial search).  The optimal for 2 is bla, for 3 is bleh, and then get to what the case study is actually about.  Now we vary the parameters $\lambda$, $\rho$, $t$, and $v$ to investigate how our recovery conditions are affected.  Compactify the actual sections and take out what's common and put that up here.  Make each of 2-sparse and 3-sparse one paragraph, and then make clear that the last paragraph is a comment on the whole thing.}
%\todo{Change subsections to Controller with 2 actuators, or something like that, and update remaining section accordingly.}
%\subsubsection*{2-atom-sparse controller}

%Our goal is to evaluate whether a desired controller with 2-atom-sparse support can be recovered by solving a truncated RFD optimization \eqref{eq:Topt}.  In particular, we seek a controller that satisfies\footnote{Here we mean that the first and fifth rows are non-zero in $U_*$.} $\A_* = \{1,5\}$, which can be verified (via exhaustive search) to be the atomic support of the 2-atom-sparse controller that minimizes a $\Htwo$ cost.  In particular, we take $U_*$ to be 
%\begin{equation}
%\begin{array}{rl}
%U_* := \argmin{U \in \RHinf}&\Htwonorm{Y-\M(U)}^2 + .1\Htwonorm{U}^2 \\
%\text{s.t.} & \left| \gsupp{U} \right| \leq s,
%\end{array}
%\label{eq:chainUs}
%\end{equation}
%with $Y$ and $\M$ as defined after \eqref{eq:h2_mm} and $s=2$.  For this $\A_*$ and system, $\tau_{\Gs} = 4$.
%
%\todo{change from $t$ varying to $t \in \left[...\right]$.}
We begin by examining how the lower bound parameter $\gtv$ and the {maximum gain} $\btv$ are affected as we vary the horizon $t$ and the controller order $v$.  In particular, for actuation sparsity $s=2$, we compute $\gtv$ and $\btv$ for (i) $t=6$ and $v\in\left\{1,\dots, 3\right\}$ (shown in Figure \ref{fig:GamBeta}),  (ii) for $v=1$ and $t\in\left\{1,\dots,4\right\}$ (shown in Figure \ref{fig:fixedV}), and (iii) for $v=2$ and $t\in\left\{2,\dots,8\right\}$ (shown in Figure \ref{fig:fixedV2}).  As expected, there is a decrease in the lower bound parameter $\gtv$ and an increase in the maximum gain $\btv$ as $v$ increases, while both $\gtv$ and $\btv$ are non-decreasing for a fixed controller order $v$ and increasing horizon $t$ as long as $t \leq \mix$. For this problem, the mixing time $\mix=5$.  Further we see that $\gtv$ begins to decrease for horizons $t> 6$ when $v=2$.

\begin{figure*}
 \begin{subfigure}{.5\columnwidth}
\includegraphics[width = \columnwidth]{gambetasmal}%
\caption{ Fixed horizon $t=6$.}%
\label{fig:GamBeta}%
\end{subfigure} \hfill %
\begin{subfigure}{.5\columnwidth}
\includegraphics[width = \columnwidth]{fixedVsmall}%
\caption{Fixed controller order $v=1$.}%
\label{fig:fixedV}%
\end{subfigure}\hfill%
\begin{subfigure}{.5\columnwidth}
\includegraphics[width = \columnwidth]{fixedV2small}%
\caption{Fixed controller order $v=2$.}%
\label{fig:fixedV2}%
\end{subfigure} \hfill%
\caption{Behavior of identifiability parameters $\gtv$ and $\btv$.}
\end{figure*}

%The fact that our sufficient conditions are only useful for $V=1$ should not be seen as discouraging.  First, we know that our bounds on $\alpha$ and $\beta$ are in general conservative for $V>2$.  Secondly and more importantly, 

The conditions of Theorem \ref{thm:main} are satisfied for $v=1$ and several values of $t$.  For example, if we select $t=4$, $v=1$, $\rho = 0$ and $U_*$ as defined in \eqref{eq:chainUs}, we can compute $(\gamma^{\leq 4,1}-\beta^{\leq 4,1})^{-1}=.7273$, $\SNR{(U^{\leq 1}_*)_1} = .7324$, and $\SNR{(U^{\leq 1}_*)_5} = .7353$, thus satisfying condition \eqref{eq:main} for each of the two actuators.  Further, selecting $\lambda=2.0119 \in \Lambda$, and using this value for $\lambda$ in the truncated RFD optimization \eqref{eq:Topt} recovers a solution with non-zero first and fifth rows.  


%Further, we verified that $\Gdnorm{\Delta} = 1.006$, which is less than the right hand side of \eqref{eq:bounded}, which was computed to be $1.12$. 

Perhaps surprisingly, similar positive recovery results can be verified for all $2\leq t \leq \mix$ -- the relevant values are summarized in Table \ref{tab:chain2sparse}.  In this table, $\text{SNR}_i$ corresponds to the SNR achieved by the controller component corresponding to the actuator at node $i$. Further, $\Delta := {\hat{U} - U^{\leq v}_*}$ is the approximation error between the architect parameter $\hat{U}$ and underlying parameter $U^{\leq v}_*$, and the values in the ``Bound'' column are given by equation \eqref{eq:bounded} in the appendix giving upper bounds on $\Gdnorm{\Delta}$.  It is worth noting that for $t=5$, we do not satisfy the sufficient conditions of Theorem \ref{thm:main}, but nonetheless recover the correct actuation architecture.  \edit{As the horizon $t$ and controller order $v$ are chosen empirically in practice, it is promising that our sufficient conditions are satisfied for a range of small values of $t$ and $v$.}

\begin{table}[h]
\centering
\begin{tabular}{c|cccccc}
\hline
 $t$ &  $\frac{1}{\gamma-\beta}$ & $\text{SNR}_1$ & $\text{SNR}_5$ & $\lambda$ &  $\Gdnorm{\Delta}$ & Bound \\ \hline
 2 & 1 & 1.27 & 1.27 & .8 & .73 & .89  \\ \hline
3&  .8 & .87 & .88 & 1.46 & .91 & 1.03 \\ \hline
 4 & .727 & .732 & .735 & 2.01 & 1.00 & 1.12  \\ \hline
5 & .7 & .67 & .68 & 2.45 & 1.05 & 1.16  \\ \hline
\end{tabular}
\caption{Summary of relevant values for the controller $U_2$ with actuators at nodes 1 and 5.}
\label{tab:chain2sparse}
\end{table}

%Now consider the goal of recovering the actuation architecture of $U_3$ via the truncated RFD optimization \eqref{eq:Topt} that satisfies $\A_* = \{1,5,9\}$, which can be verified (once again via exhaustive search) to be the group support of the 3-atom-sparse controller that minimizes the LQR cost \eqref{eq:chainUs}. \todo{this will be moved up}

We now consider the case of actuation sparsity $s=3$. Much as in the $s=2$ case, we can verify that the conditions of Theorem \ref{thm:main} hold for $v=1$, and $2\leq t \leq \mix$, where the mixing time $\mix$ is still 5.  However, since the controller with 3 actuators is able to achieve a much better closed loop norm, the SNRs are significantly larger, while the SNR threshold $(\gtv-\btv)^{-1}$ does not change significantly. In particular, for the case of $t=5$, we have a threshold of $(\gamma^{\leq 5,1}-\beta^{\leq 5,1})^{-1}=.82$, and SNRs of $4.04$, $4.04$ and $2.67$ for the three actuator components.  

This is consistent with our original interpretation of $\wt$, the closed loop response of the system, playing the role of measurement noise -- the better the performance of the controller, the easier it is to identify via RFD.  In general, these experiments demonstrate that controllers with sparse and diffuse actuations schemes that achieve a small closed loop performance $\wt$ are easy to identify as the solutions to RFD optimization problems.  In summary, our analysis and case studies demonstrate that:
\begin{itemize}
\item   The parameter $\rho$ can be set to 0 in the RFD optimization problem \eqref{eq:rfd_opt}, even if the original model matching problem \eqref{eq:gen_mm} had non-zero control cost $\rho_u$.
%\item Structure, rather than randomness, leads to identifiability in control.
\item Choosing small controller order $v$ and horizon $t$ can actually lead to a favorable threshold $(\gtv - \btv)^{-1}$ \eqref{eq:main}.
\item Actuation schemes that are more evenly distributed (so that they lead to large mixing times $\mix$ in \eqref{eq:tau}) are easier to identify.
\item Controller components that maximize the RFD analog of a SNR \eqref{eq:groupSNR} are more likely to satisfy our recovery conditions.  In particular, these consist of controllers that have a concentration of energy in their early impulse response elements, and that achieve a small closed loop norm.
\end{itemize}



%\subsection{Unstable Symmetric Ring System}
%\todo{add a note that we consider a finite horizon 
%In this section, we consider a ring system that is symmetric and has unstable open loop dynamics.  In particular, we have $B_2 = C_1 = I_{12}$, $A = .75 I_{12} + .5 Z_{12} - .5 Z_{12}^\top$,  $B_1 = .1I_{10} + .15(E_1 + E_5 + E_9)$, $\rho_u = 1$ and we optimize over a horizon of $n=50$.  In particular, notice that $A$, $B_2$, and $C_1$ are circulant matrices, that the system is open-loop unstable as $|\lambda_{\max}(A)|=1.25$, and that $B_1$ is invariant under permutations of $\{1,5,9\}$.  
%
%%Despite the fact that this system is extremely symmetric in its parameters, there are underlying asymmetries introduced into $\M$ due to the causal nature of the system.  
%As such, we are still able to compute that, for example, $t=2$, $v=1$ and $\rho = 0$, the 3-atom-sparse controller, with $\A_* = \{1, 5, 9\}$, defined by
%\begin{equation}
%\begin{array}{rl}
%U_* := \argmin{U \in \RHinf}&\Htwonorm{Y-\M(U)}^2 + \Htwonorm{U}^2 \\
%\text{s.t.} & \left| \gsupp{U} \right| \leq 3,
%\end{array}
%\label{eq:chainUs}
%\end{equation}
%satisfies our sufficient conditions.  In particular, we find that $(\gamma^{\leq 2,1}-\beta^{\leq 2,1})^{-1} = .64$, whereas the SNR of all groups was computed to be $.68$.

%\todo{add a punchline}
%Thus, despite a significant degree of symmetry in this unstable system, optimizing over the horizon of $t=2$ with a controller approximation of order $v=1$ is provably sufficient to recover the support of the optimal 3-atom-sparse controller.



%As remarked in the previous section, using the bound $\eqref{eq:alpha}$ implies that we need the stronger condition that $\gamma > \beta$ for our sufficient conditions to be useful.  Using \eqref{eq:alpha_bound} and \eqref{eq:beta_bound}, a condition sufficient for this to hold is that
%\begin{equation}
%\max_{j \in \Gs^\perp} \sum_{g\in\Gs}\sigma_{jg} <  \max_{j\in J} \left\{\underline{\sigma}_j - \sum_{g\neq j \in J} \sigma_{jg} \right\}
%\end{equation}
%for all $J \subseteq \Gs$, where, to lighten notational burden, we have let
%\begin{equation}
%\underline{\sigma}_j :=  \sm{S_j^\dag S_j}
%\end{equation}
%and
%\begin{equation}
%\sigma_{jg} = \sM{S_j^\dag S_g}.
%\end{equation} 
%
%In other words, these quantities are functions of the open-loop plant and $T$ -- this subsection will explore how the choice of $T$ can affect these parameters, and show perhaps somewhat counter-intuitively, it is often beneficial to truncate the RFD optimization to a small $T$.  The key piece of intuition to keep in mind throughout the section is that we are looking to recover the \emph{structure} of $U^*$, rather than its actual values (as these can be found via a polishing step), and that structure is \emph{invariant} under truncation in time.
%
%As neither $\lambda$ nor $\rho$ appear in these expressions, our only tuning parameter that affects these quantities is $T$ -- how it does so will be explored next.  



==> conclusion.tex <==
%In this paper we presented RFD as a natural synthesis of approximation theory and optimal control.  In particular, we augmented traditional and distributed model matching problems with suitable penalties so that a structured controller is found, where this structure has a direct interpretation in terms of the controller's actuation, sensing and communication architectures.
%
%Further, we described natural connections between structured inference and structured controller synthesis problems. By appropriately interpreting the open-loop response, the map from control to closed loop response, and the closed loop response in the context of structured approximation, we were able to show that {convex} RFD optimizations with atomic norm regularizers enjoy the same theoretical guarantees as their structured inference counterparts.  Specifically, if certain identifiability and SNR conditions hold then computationally tractable convex programming, performed over a finite horizon with a low-order controller, can be used to identify optimal controller architectures.
%
%Directions for future work include:
%\noindent\textbf{Overlapping Atoms}:  Extending the analysis in Section \ref{sec:recovery} to the case where the support of the atoms are allowed to overlap is important.  In particular, problems involving the simultaneous placement of sensors and actuators, as well as the design of information sharing constraints in the context of distributed control, all involve atoms with overlapping support.  The challenge is that when we allow such an overlap, identifiability conditions such as those that we relied  on in our analysis do not hold.

\noindent\textbf{Alternative performance metrics}: Our analysis has focused on the $\h_2$/LQG performance metrics because of their direct connection to regularized least squares problems such as those considered in \cite{CRPW12}.  In future work, we plan to explore connections between minimax structured inference and $\h_\infty$ and $\mathcal{L}_1$ optimal and robust control, in order to expand the scope of RFD optimization, and to make deeper connections to the statistical inference literature.

\noindent\textbf{A priori bounds on incoherence}: It is of great interest to derive \apriori \ bounds on the gain parameters $\atv$ \eqref{eq:alpha} and $\btv$ \eqref{eq:beta} in terms of the state-space parameters of the system and a lower bound on the mixing time $\mix$ \eqref{eq:tau}.  This would allow for broader classes of systems to be classified as being amenable to RFD. \edit{Inspired by semidefinite relaxation approaches to computing restricted isometry constants \cite{d2007direct},we are currently pursuing computationally tractable methods to obtain bounds on these parameters \cite{YM_CDC15}.}

%\noindent\textbf{Specialized solvers}: A vast array of specialized solvers exists for SLIP problems that use the atomic norms that we have described.  Although these can be readily ported as is, it is of interest as to whether they can be further accelerated by exploiting the block lower-triangular Toeplitz structures that arise due to the LTI nature of the underlying operators.

\noindent\textbf{Connections to other convex controller synthesis frameworks}: Recently, it has been shown that for positive systems \cite{TL11,R12}, for alternative cost functions \cite{DTF13}, and for localized optimal control \cite{WMYD_ACC14,WMD_CDC14,WM_Allerton14},  structured optimal \emph{linear} controllers can be computed via convex optimization -- it is of interest to extend the RFD framework to accommodate such synthesis methods as well.

==> introduction.tex <==
%As we move into the era of large scale systems, such as the new smart grid, clean slate internet and automated highway systems, the design of control systems will become increasingly challenging.  Indeed, it will no longer be possible to take for granted the existence of a control architecture: placing sensors \& actuators, as well as the communication links between them, will become an integral part of the design process, in addition to the traditional design of the control laws themselves.

As we move into the era of large-scale systems such as the smart-grid, software defined networking and automated highways, the design of control systems is becoming increasingly more challenging.  Designing the controller \emph{architecture} -- placing sensors and actuators as well as the communication links between them -- is now as important as the traditional design of the control laws themselves.

A conceptually useful viewpoint in the design of controller architectures is to consider complicated systems as being composed of multiple simpler \emph{atomic} subsystems.  For example, if the task is to design the actuation architecture of a controller, a natural atomic element is a controller with a single actuator -- it is then clear that a general architecture can be built out of such atoms.  In general, controllers with a dense actuation, sensing and communication architecture (i.e., systems that consist of many atomic subsystems) achieve better closed loop performance in comparison with those with sparse architectures (i.e., systems composed of a small number of atomic subsystems).  However, as these architectural resources translate into actual hardware requirements, it is desirable from both a maintenance and a cost perspective that we minimize the total number of atomic elements used.  Hence, the problem of controller architecture/control law co-design is one of jointly optimizing an appropriately defined structural measure of the controller and its closed loop performance by trading off between these two competing metrics in a principled manner.  In other words, we seek an approximation of a given optimal controller by one that utilizes fewer atomic elements without a significant loss in performance.  This goal has parallels with the approximation theory literature in which one seeks approximations of complicated functions as combinations of elements from a simpler class of functions such as the Fourier basis or a wavelet basis \approxcitations.

In an appropriate parameterization, pure controller synthesis methods in a model matching framework can be interpreted as techniques for solving a particular linear inverse problem in which one is given an open loop response of a system $Y$ and a linear map $\Cl$ from the controller to the closed loop response, and one seeks a controller $U$ such that \edit{$Y - \Cl(U) \approx 0$} (as measured in a suitable performance metric).  From this perspective, our objective in joint controller architecture/control law co-design is to obtain \emph{structured} solutions to the linear inverse problem underlying controller synthesis.  Such \emph{structured linear inverse problems} (SLIP) are of interest in diverse applications across applied mathematics -- for instance, computing sparse solutions to linear inverse problems or computing low-rank solutions to systems of linear matrix equations arise prominently in many contexts in signal processing and in statistics \ellcitations, \nuccitations.  

In these problem domains, minimizing the $\ell_1$ norm subject to constraints described by the specified equations is useful for obtaining sparse solutions \ellcitations, and similarly, nuclear norm minimization is useful for obtaining low-rank solutions to linear matrix equations \nuccitations.  These ideas were extended in \cite{CRPW12}, where the authors describe a generic convex programming approach -- based on minimizing an appropriate \emph{atomic norm} \approxcitations  -- for inducing a desired type of structure in solutions to linear inverse problems.  Motivated by these developments, our approach to the problem of joint architecture/control law co-design is to augment variational formulations of traditional controller synthesis methods with suitable convex regularization functions.  The role of these regularizers is to penalize controllers with more complex architectures in favor of those with less complex ones, thus inducing controllers with a simpler architecture.  We call this framework \emph{Regularization for Design} (RFD).


%We refer the interested reader to \cite{W14} for a review of the current state of the art, both theoretically and computationally, of using regularizers to induce structure in a statistical setting.

%From this perspective, the problem of joint architecture/contol law co-design can be viewed as one of approximating a given optimal controller by a simpler controller consisting of a smaller number of our objective is to find an approximation of a given optimal controller that judiciously utilizes a limited set of available architectural resources.


%A natural approach to such a structured approximation problem is to add a discrete penalty that counts the number of architectural elements being used.  Although intuitively appealing, the inclusion of a discrete penalty brings the co-design procedure into the realm of combinatorial optimization, and as such leads to what are in general computationally intractable problems.  Similar combinatorial optimizations, in which one seeks to trade-off between a traditional and structural metric, arise frequently in the context of structured inference problems.  Rather than attempting to solve the combinatorial optimization directly, a successful approach in this setting has been to replace the discrete penalties with suitable convex relaxations in order to provably recover desirable structured solutions.


%In particular, in inference problems, it is often known
%\emph{a priori} that the desired model should
%be structurally ``simple.''  Subject to certain technical conditions on the measurements taken, it has been shown that simple structure can often be approximately, and sometimes exactly, recovered by minimizing
% an appropriately chosen convex penalty function.

\textbf{Related Work:} Regularization techniques based on $\ell_1$ norms and, more generally, atomic norms have already been employed extensively in system identification, e.g., to identify systems of small Hankel order (cf. \cite{SBTR12,Fazel,MR_CDC14}), and in linear regression based methods \cite{LjungNewOld}.  Although the resulting solutions yield structured systems, they typically do not have a direct interpretation in terms of the architecture of a control system (i.e., actuators, sensors and the communication links between them).  The use of regularization explicitly for the purpose of designing the architecture of a controller can also be found in the literature.  Examples include the use of $\ell_1$ regularization to design sparse structures in $\mathcal{H}_2$ static state feedback gains \cite{LFJ13}, treatment therapies \cite{JRM14}, synchronization \cite{FLJ13} topologies; the use of group norm penalties to design actuation/sensing schemes \cite{MC_CDC14,DJL14}; and the use of a specialized atomic norm to design communication delay constraints that are well-suited to $\mathcal{H}_2$ distributed optimal control \cite{M_CDC13_codesign, M_TCNS14}.  Although these methods provide an algorithmic approach for designing controllers with a desired architecture in certain specialized settings, they do not enjoy the same theoretical support that regularization techniques for structured inverse problems enjoy in other settings \approxcitations, \ellcitations, \nuccitations.  \edit{It is also worth noting that methods have been developed to identify minimal architectures that guarantee the structural observability and controllability of a system \cite{PKP15}.}

%I want to say something along the lines of... but a little softer
%The structured controller synthesis methods presented in \cite{LFJ13,DLFM12} are inherently non-convex, even without the regularizer.  In particular this means that even once a suitable architecture has been identified, it is in general not possible to find the optimal controller with underlying structure defined by that architecture.  Further, although \cite{LFJ13,DLFM12,FLJ13,DJL14} claim to identify optimal controller architectures, the only proof that they provide for this claim is the use of a sensible convex relaxation to a cardinality like penalty.


\textbf{Our Contributions:} 
\edit{This paper presents significant computational and theoretical contributions to the area of joint optimal controller architecture/control law co-design.  From a computational perspective, we propose a general RFD framework that is applicable in a much broader range of settings than the previous approaches mentioned above.  We restrict ourselves to problems for which the linear optimal \note{structured} controller is specified as the solution to a convex optimization problem \cite{RL06,RCL10,LL11_QI}.  As a result, RFD optimization problems with convex regularization functions are convex programs and consequently, for many cases of interest, the optimal linear structured controller restricted to the designed architecture can be computed exactly, e.g., \distcitations.   Specifically:
\begin{itemize}
\item We provide a catalog of atomic norms useful for control architecture design.  In particular, in addition to known penalties for actuator, sensor and communication design, we provide novel penalties for \emph{simultaneous} actuator, sensor and/or communication design.
\item We describe a unifying framework for RFD that encompasses state and output feedback problems in centralized and distributed settings, and in which any subset of actuation, sensing, and/or communication architectures are co-designed.
\item We define a two step algorithm that first identifies the controller architecture via a finite-dimensional convex RFD optimization problem, and then solves for the potentially infinite dimensional linear optimal controller restricted to the designed architecture using methods from classical and distributed optimal control \distcitations.
\end{itemize}
%\note{This ensures that once a controller architecture is identified through the solution to a RFD optimization problem, the globally optimal controller with underlying structure restricted to that architecture can then be solved for.  This is in contrast to the methods presented in \cite{LFJ13,DLFM12} which are built around inherently non-convex optimization problems, regardless of the penalty function used.}
To provide theoretical support to our proposed computational framework, we make explicit links between RFD optimization problems and the use of convex optimization in structured inference problems.  We build on these links to analyze the properties of structured controllers generated by RFD synthesis methods, which leads to conditions under which RFD methods succeed in identifying optimally-structured controllers.  
%\note{We provide a rigorous proof that convex regularization functions can be used to identify optimally-structured controllers. Once again, this is in contrast with \cite{LFJ13,DLFM12,FLJ13,DJL14} in which the authors implicitly claim that optimality of the identified controller structure follows immediately from using sensible convex regularization functions -- this is simply not the case.}
We prove that convex regularization functions can be used to identify
optimally-structured controllers; our analysis and results are natural
control-theoretic analogs of similar results in the statistical
inference literature.
Specifically:}
%% In order to do so, we develop control theoretic analogs to SLIP identifiability conditions and signal to noise ratios (SNRs), and argue that \emph{identifying} suitably structured estimators in SLIP is in fact mathematically parallel to \emph{designing} suitably structured controllers in an optimal control setting.  We re-interpret the parameters and measures of success of SLIP to be compatible with RFD, and leverage analysis methods from the structured inference literature to gain insight into the properties of the co-designed controller.
\edit{
\begin{itemize}
\item We show that by varying the regularizer used, we recover control-theoretic analogs to prominent approaches in statistical modeling such as Ordinary Least Squares, Ridge Regression \cite{Ridge}, Group Lasso \cite{GroupLasso}, and Group Elastic Net \cite{ElasticNet}.
\item We show that finite-horizon finite-order convex approximations of an RFD optimization problem can recover the structure of an underlying infinite dimensional optimal controller.
\item We define control-theoretic analogs of identifiability conditions and signal-to-noise ratios (SNRs), and we provide sufficient conditions based on these for a control architecture to be identified by RFD.  In particular we show that controllers that maximize this SNR like quantity are more easily recovered via RFD than those that do not.
\item We provide a concrete example of a system satisfying the above identifiability and SNR conditions.  In particular, this is the first system in the literature for which it is shown that convex optimization provably recovers the actuation architecture of an underlying optimally structured controller.
\end{itemize}}

%By exploiting the connection to SLIP, we provide theoretical analysis support of our methods (i.e., conditions under which optimally structured controllers are  underfor In particular, in SLIP, exact or approximate recovery of an underlying desired model can be guaranteed subject to certain identifiability conditions -- these conditions also inform the properties one expects the solutions of such optimizations to have.  To the best of our knowledge, no such guarantees exist in the context of RFD, despite the vast amount of empirical evidence that these methods yield structured controllers with desirable properties.
%
%
%Although these previous methods provide an algorithmic approach to designing controllers with a desired architecture in certain specialized settings, they do not enjoy the type of theoretical support preform a computational link between sparse reconstruction theory and control architecture co-design.  The algorithmic methods have been ported, with great success, but these methods do not yet enjoy the same theoretical support that their sparse reconstruction counterparts do.  
%


\textbf{Paper Organization}: \edit{In Section \ref{sec:prelims}, we define notation and discuss the relevant concepts from operator theory.  This paper is then organized in a modular fashion: Sections \ref{sec:RFD} through \ref{sec:rfd_proc} focus on the computational aspects of controller architecture design, whereas Sections \ref{sec:recovery} and \ref{sec:case} focus on conditions for optimal architecture recovery.  Specifically, in Section \ref{sec:RFD}, we introduce the RFD framework as a natural blend of controller synthesis methods and regularization techniques.  In Section \ref{sec:RFD_algos}, we focus on RFD problems with an $\Htwo$ performance metric and an atomic norm penalty; we present a catalog of atomic norms that are useful for controller architecture design, and make connections to the structured inference literature.  The computational component of the paper concludes in Section \ref{sec:rfd_proc}, in which we formally define the two-step RFD procedure, and apply the RFD framework to a simultaneous actuator, sensor and communication design problem. .  In Section \ref{sec:recovery}, we shift to a more theoretical discussion:  we make connections between structured controller approximation and structured inference problems by framing both tasks as finding structured solutions to linear inverse problems, and leverage these connections to describe interpretable sufficient conditions for the success of a finite-dimensional RFD optimization problem.  In Section \ref{sec:case}, we provide a case study to further illustrate the applicability of these results, and summarize the prior development.  Finally, we conclude with a discussion of directions for future work Section \ref{sec:conclusion}.}


==> large.tex <==

In this subsection we demonstrate the full power and flexibility of the RFD framework in designing a distributed controller architecture, jointly incorporating actuator, sensor and communication link design.  In particular we consider a plant with eleven subsystems with topology as illustrated in Figure \ref{fig:RFD_topo}.  The solid lines correspond to the physical interconnection between subsystems. Choosing $C_2 = B_2 = I$, the adjacency matrix of this graph then defines the support of the $A$ matrix in the state space realization 
%(shown in equation \eqref{eq:Amatrix}) 
of the generalized plant \eqref{eq:genplant}, as well as the required communication links between nodes such that the distributed constraint is QI under $P_{22}$ \cite{M_TCNS14,RCL10}. 

%\begin{equation}
%A = \left[\begin{array}{ccccccccccc}  \ast  &       0  & \ast   &      0     &    0    &     0    &     0     &    0    &     0     &    0    &     0 \\
%         0   &  \ast   & \ast    &    0    &     0     &    0   &      0     &    0    &     0    &     0    &     0 \\
%    \ast   & \ast &   \ast &   \ast   &       0    &     0    &     0     &    0     &    0     &    0     &    0\\
%         0      &   0 &   \ast &   \ast &  \ast   &\ast&   \ast  &      0       &  0    &     0     &    0\\
%         0     &    0    &     0  & \ast&   \ast  &     0    &     0     &    0    &     0      &   0       &  0\\
%         0       &  0   &      0  & \ast   &      0  & \ast   &      0   &      0     &    0     &    0    &     0\\
%         0      &   0   &      0  &  \ast   &     0   &      0 &   \ast  &  \ast &   \ast &      0    &     0\\
%         0     &    0      &   0    &     0     &    0   &      0 &  \ast&   \ast  &      0    &     0      &   0\\
%         0      &   0    &     0  &       0    &     0    &     0 &   \ast &        0  &  \ast&  \ast &  \ast\\
%         0       &  0   &      0    &     0     &    0    &     0    &     0   &      0 &   \ast &  \ast  &       0\\
%         0      &   0     &    0     &    0     &    0    &     0   &      0   &      0 & \ast  &       0  &  \ast   \end{array}\right]
%         \label{eq:Amatrix}
%\end{equation}

\begin{figure}[h!]
\centering
\includegraphics[width = .35\textwidth]{RFD_topo}
\caption{Topology of system considered for RFD example.  Solid lines indicate both physical interconnections and existing communication links between controllers.  Dashed lines correspond to possible additional edges to be added.  %Further each node can be equipped with a sensor and an actuator.  The resulting space of actuator/sensor/communication topologies contains 536,870,911 different possible combinations.
}
\label{fig:RFD_topo}
\end{figure}
\vspace{-1mm}
The non-zero entries of $A$ were generated randomly and normalized such that $|\lambda_{\max}\left(A\right)|=.999$. The remaining state space parameters of the generalized plant \eqref{eq:genplant} satisfy $D_{12}\begin{bmatrix} C_1^\top & D_{12}^\top \end{bmatrix} =  \begin{bmatrix} 0 & 25 I \end{bmatrix}$, and $D_{21}^\top\begin{bmatrix} B_1 & D_{21} \end{bmatrix} =  \begin{bmatrix} 0 & .01 I \end{bmatrix}$, with $C_1C_1^\top = 100 I$ and $B_1^\top B_1 = I$.

For the RFD task, we choose an $\Htwo$ norm performance metric; we allow each node to be equipped with an actuator and/or a sensor (for a total of 11 possible actuators and sensors), and we allow the communication graph to be augmented with any subset of the interconnections denoted by the dashed lines in Figure \ref{fig:RFD_topo}, in addition to the already present links given by the solid lines.  This leads to 536,870,911 different possible controller architectures.

\note{We solved the RFD optimization \eqref{eq:output} with atomic norm $\norm{\cdot}_{\text{act+sns+comm}}$ as defined in \S\ref{sec:atoms}, with weighting parameter $\theta = .75$ and with $k_s = k_a = 1$.   We chose a horizon $t=8$, a controller order $v=4$, and set $\rho = 0$. We vary $\lambda$, and for each resulting optimal solution, we identified the designed architecture.  We then used the method from \cite{LD14, LDXX} to exactly solve the resulting non-regularized distributed $\Htwo$ model matching problem restricted to the architecture underlying $\tilde{U}$.  Note that the Youla parameter solving this non-regularized problem is not restricted to have a finite impulse response.  In particular, we can compute the optimal Youla parameter and the corresponding optimal controller restricted to the architecture underlying $\tilde{U}$ in a computationally tractable fashion because we guarantee that the subspace corresponding to the designed architecture is QI, as per the discussion in Section \ref{sec:RFD_algos}.}

The resulting architectural complexity is plotted against the closed loop norm of the system in Figure \ref{fig:rfd_perf}.  As $\lambda$ is increased, the architectural complexity (i.e. the number of actuators, sensors and communication links) decreases, but at the expense of deviations from the performance achievable by the controller that uses all of the available architectural resources.  We also show the resulting architecture for $\lambda = 200$ in Figure \ref{fig:designed}: as can be seen, a non-obvious combination of six actuators, nine sensors and three additional communication links are chosen, resulting in only a 0.27\% degradation in performance over the distributed controller using all eleven actuators, eleven sensors and seven additional communication links.

\begin{figure}[h!]
\centering
\includegraphics[width = .35\textwidth]{large_plot}
\caption{A small degradation in closed loop performance allows for a significant decrease in architectural complexity.}
\label{fig:rfd_perf}
\end{figure}

%\begin{figure}[h!]
%\centering
%\includegraphics[width = .35\textwidth]{perf}
%\caption{As $\lambda$ is increased, the performance of the system degrades.}
%\label{fig:perf}
%\end{figure}

\begin{figure}[h!]
\centering
\includegraphics[width = .35\textwidth]{designed}
\caption{Resulting architecture for $\lambda=200$: despite only using six actuators (orange squares), nine sensors (blue triangles) and three additional communication links (green arrows), the performance only degraded by 0.27\% relative to  the distributed controller using all eleven actuators, eleven sensors and seven communication links.}
\label{fig:designed}
\end{figure}





==> large_abr.tex <==

In this subsection we demonstrate the full power and flexibility of the RFD framework in designing a distributed controller architecture, jointly incorporating actuator, sensor and communication link design.  In particular we consider a plant with eleven subsystems with topology as illustrated in Figure \ref{fig:RFD_topo}.  The solid lines correspond to the physical interconnection between subsystems. Choosing $C_2 = B_2 = I$, the adjacency matrix of this graph then defines the support of the $A$ matrix in the state space realization 
%(shown in equation \eqref{eq:Amatrix}) 
of the generalized plant \eqref{eq:genplant}, as well as the required communication links between nodes such that the distributed constraint is QI under $P_{22}$ \cite{M_TCNS14,RCL10}. 

%\begin{equation}
%A = \left[\begin{array}{ccccccccccc}  \ast  &       0  & \ast   &      0     &    0    &     0    &     0     &    0    &     0     &    0    &     0 \\
%         0   &  \ast   & \ast    &    0    &     0     &    0   &      0     &    0    &     0    &     0    &     0 \\
%    \ast   & \ast &   \ast &   \ast   &       0    &     0    &     0     &    0     &    0     &    0     &    0\\
%         0      &   0 &   \ast &   \ast &  \ast   &\ast&   \ast  &      0       &  0    &     0     &    0\\
%         0     &    0    &     0  & \ast&   \ast  &     0    &     0     &    0    &     0      &   0       &  0\\
%         0       &  0   &      0  & \ast   &      0  & \ast   &      0   &      0     &    0     &    0    &     0\\
%         0      &   0   &      0  &  \ast   &     0   &      0 &   \ast  &  \ast &   \ast &      0    &     0\\
%         0     &    0      &   0    &     0     &    0   &      0 &  \ast&   \ast  &      0    &     0      &   0\\
%         0      &   0    &     0  &       0    &     0    &     0 &   \ast &        0  &  \ast&  \ast &  \ast\\
%         0       &  0   &      0    &     0     &    0    &     0    &     0   &      0 &   \ast &  \ast  &       0\\
%         0      &   0     &    0     &    0     &    0    &     0   &      0   &      0 & \ast  &       0  &  \ast   \end{array}\right]
%         \label{eq:Amatrix}
%\end{equation}

\begin{figure}[h!]
\centering
\includegraphics[width = .25\textwidth]{RFD_topo}
\caption{Topology of system considered for RFD example.  Solid lines indicate both physical interconnections and existing communication links between controllers.  Dashed lines correspond to possible additional edges to be added.  %Further each node can be equipped with a sensor and an actuator.  The resulting space of actuator/sensor/communication topologies contains 536,870,911 different possible combinations.
}
\label{fig:RFD_topo}
\end{figure}
\vspace{-1mm}
The non-zero entries of $A$ were generated randomly and normalized such that $|\lambda_{\max}\left(A\right)|=.999$. The remaining state space parameters of the generalized plant \eqref{eq:genplant} satisfy $D_{12}\begin{bmatrix} C_1^\top & D_{12}^\top \end{bmatrix} =  \begin{bmatrix} 0 & 25 I \end{bmatrix}$, and $D_{21}^\top\begin{bmatrix} B_1 & D_{21} \end{bmatrix} =  \begin{bmatrix} 0 & .01 I \end{bmatrix}$, with $C_1C_1^\top = 100 I$ and $B_1^\top B_1 = I$.

For the RFD task, we choose an $\Htwo$ norm performance metric; we allow each node to be equipped with an actuator and/or a sensor (for a total of 11 possible actuators and sensors), and we allow the communication graph to be augmented with any subset of the interconnections denoted by the dashed lines in Figure \ref{fig:RFD_topo}, in addition to the already present links given by the solid lines.  This leads to 536,870,911 different possible controller architectures.

\note{We solved the RFD optimization \eqref{eq:output} with atomic norm $\norm{\cdot}_{\text{act+sns+comm}}$ as defined in \S\ref{sec:atoms}, with weighting parameter $\theta = .75$ and with $k_s = k_a = 1$.   We chose a horizon $t=8$, a controller order $v=4$, and set $\rho = 0$. We vary $\lambda$, and for each resulting optimal solution, we identified the designed architecture.  We then used the method from \cite{LD14} to exactly solve the resulting non-regularized distributed $\Htwo$ model matching problem restricted to the architecture underlying $\tilde{U}$.  Note that the Youla parameter solving this non-regularized problem is not restricted to have a finite impulse response.  In particular, we can compute the optimal Youla parameter and the corresponding optimal controller restricted to the architecture underlying $\tilde{U}$ in a computationally tractable fashion because we guarantee that the subspace corresponding to the designed architecture is QI, as per the discussion in Section \ref{sec:RFD_algos}.}

The resulting architectural complexity is plotted against the closed loop norm of the system in Figure \ref{fig:rfd_perf}.  As $\lambda$ is increased, the architectural complexity (i.e. the number of actuators, sensors and communication links) decreases, but at the expense of deviations from the performance achievable by the controller that uses all of the available architectural resources.  We also show the resulting architecture for $\lambda = 100$ in Figure \ref{fig:designed}: as can be seen, a non-obvious combination of six actuators, nine sensors and three additional communication links are chosen, resulting in only a 0.27\% degradation in performance over the distributed controller using all eleven actuators, eleven sensors and seven additional communication links.

\begin{figure}[h!]
\centering
\includegraphics[width = .3\textwidth]{large_plot}
\caption{A small degradation in closed loop performance allows for a significant decrease in architectural complexity.}
\label{fig:rfd_perf}
\end{figure}

%\begin{figure}[h!]
%\centering
%\includegraphics[width = .35\textwidth]{perf}
%\caption{As $\lambda$ is increased, the performance of the system degrades.}
%\label{fig:perf}
%\end{figure}

\begin{figure}[h!]
\centering
\includegraphics[width = .25\textwidth]{designed}
\caption{Resulting architecture for $\lambda=100$: despite only using six actuators (orange squares), nine sensors (blue triangles) and three additional communication links (green arrows), the performance only degraded by 0.27\% relative to  the distributed controller using all eleven actuators, eleven sensors and seven communication links.}
\label{fig:designed}
\end{figure}





==> rfd_algos.tex <==
In this section we examine convex formulations of the RFD optimization \eqref{eq:rfd_opt} by restricting our attention to convex cost functions $\cost{\cdot; Y, \Cl}$ and {convex} penalty functions $\Omega\left(\cdot\right)$.

\subsection{Convex Cost Functions}
\label{sec:cost_fcns}
Any suitable convex cost function $\cost{\cdot; Y, \Cl}$ can be used in \eqref{eq:rfd_opt}: traditional examples from robust and optimal control include the $\Htwo$, $\Hinf$ \cite{ZDG96} and $\mathcal{L}_1$ norms \cite{DahlehL1}.  We focus on the $\Htwo$ norm as a performance metric because it allows us to make direct connections between the RFD optimization problem \eqref{eq:rfd_opt} and well-established methods employed in statistical inference such as ordinary least squares, Ridge Regression \cite{Ridge}, Group Lasso \cite{GroupLasso} and Group Elastic Net \cite{ElasticNet}.

We begin by introducing a specialized form of the model matching problem \eqref{eq:gen_mm}, and show how state-feedback problems with $\Htwo$ performance metrics can be put into this form.

\begin{defn}
Let $U, \, Y\in\RHinf$, and $\M:\RHinf \to \RHinf$ be of compatible dimension.  The optimization problem
\begin{equation}
\begin{array}{rl}
\minimize{U\in \RHinf} & \Htwonorm{Y - \M(U)}^2+\rho\Htwonorm{U}^2\\
\text{s.t.} & U \in \s
\end{array}
\label{eq:the_opt}
\end{equation}
is the $\Htwo$ \emph{optimal control problem} for a suitable parameter $\rho$ and a distributed constraint $\s$.
\end{defn}

\edit{In this definition, $Y=C_1(zI-A)^{-1}B_1$ is the state component of the open loop response, and $\M$ is the map from the Youla parameter to state component of the closed loop response. }
%We obtain this definition by writing the open loop response $Y$ as $Y=\begin{bmatrix}X & 0\end{bmatrix}$, where $X$ corresponds to the open loop state response of the system, and $0$ to the open loop control response of the system (i.e., there is no control action in open loop).  Similarly, we write the map 
%$\Cl$ from Youla parameter $U$ to closed loop response as $\Cl =  \begin{bmatrix}\M & \rho_u I\end{bmatrix}$; here $\M$ is the map from $U$ to the state response of the closed loop system, and $\rho_u I$ is the map from $U$ to the control cost component of the closed loop response.  
Explicitly separating the cost of the state component of the closed loop response $\Htwonorm{Y - \M(U)}^2$ from the control cost $\rho\Htwonorm{U}^2$ of the closed loop response allows us to connect the $\Htwo$ {RFD optimization} to several well-established methods in the inference literature.  %We are able to separate these two components of the closed loop response due to the orthogonality assumptions made on the state space parameters of the generalized plant \eqref{eq:genplant}.
Before elaborating on some of these connections, we provide two examples of standard control problems that can be put into this form.

\begin{example}[Basic LQR]
Consider the basic LQR problem given by
\begin{equation}
\begin{array}{rl}
\minimize{u\in \ell_2} & \sum_{t=0}^\infty \|Cx_t\|_{\ell_2}^2 + \|Du_t\|_{\ell_2}^2 \\
\text{s.t.} & x_{t+1} = Ax_t + Bu_t,\ x_0 = \xi,
\end{array}
\end{equation}
and assume that $D^\top D = \rho_u I$, for some $\rho_u\geq0$.
Define $\rho = \rho_u$, $X^{(t)} = CA^{t}\xi$ for $t\geq 0$, $U^{(t)} = u_t$, and $\M(U) = -H\ast U$, where $H\in \Rp$ with $H^{(0)}=0$, and $H^{(t)} = CA^{t-1}B$ for $t\geq 1$.  We can then rewrite the basic LQR problem as
\begin{equation}
\begin{array}{rl}
\minimize{U\in \RHinf} & \Htwonorm{Y-\M(U)}^2 + \rho_u\Htwonorm{U}^2.
\end{array}
\label{eq:noreg}
\end{equation}
\label{ex:bLQR}
\end{example}

\edit{
\begin{example}[$\Htwo$ State Feedback]
Assume either that the generalized plant \eqref{eq:genplant} is open-loop stable or that the control problem is over a finite horizon.  Let $C_2 = I$ and $D_{21} =0$ in the generalized plant \eqref{eq:genplant} such that the problem is one of synthesizing an optimal state-feedback controller, and for clarity of exposition, assume that $B_1$ is invertible.\footnote{\edit{The assumption that $B_1$ is invertible simply implies that no component of the state is deterministic, and can be relaxed at the expense of more complicated formulas.}}   Define the Youla parameterization for the controller synthesis problem \eqref{eq:OC} as follows \cite{ZDG96}:
\begin{equation}
\begin{array}{rclrcl}
\tilde{P}_{12} &=& \frac{1}{z}P_{12}, &
\tilde{P}_{21} &=& AP_{21} + B_1 \\
\tilde{U}&=&K(I-P_{22}K)^{-1}\tilde{P}_{21},
\end{array}
\end{equation}
with all other parameters remaining the same.  Under this parameterization, the optimal control problem \eqref{eq:OC} (with additional QI distributed constraint $\s$) with performance metric $\Htwonorm{\cdot}^2$ can be written as
\begin{equation}
\begin{array}{rl}
\minimize{\tilde{U}\in\RHinf} & \cost{\tilde{U}; P_{11}, \M} \\
\text{s.t.} & \tilde{U}\tilde{P}_{21}^{-1} \in \s,
\end{array}
\label{eq:sf_mm}
\end{equation}
where $\M = \frac{1}{z}P_{12}$ is the map from $\tilde{U}$ to the state component of the closed loop response, and 
\begin{equation}
\cost{\tilde{U}; P_{11}, \M} := \Htwonorm{P_{11} - \M\left(\tilde{U}\right)}^2 + \rho_u\Htwonorm{\tilde{U}}^2.
\label{eq:state_cost}
\end{equation}
The optimal controller $K$ is then recovered from the solution to \eqref{eq:sf_mm} as $K=(I+\tilde{U}\tilde{P}_{21}^{-1}P_{22})^{-1}\tilde{U}\tilde{P}_{21}^{-1}$.  The state-feedback assumption and the choice of Youla parameterization ensure that $\tilde{P}_{21}$ is invertible in $\RHinf$ and that $K \in \s$.  
%We further specialize the problem by choosing $\cost{\cdot}$ to be the $\Htwo$ norm of the closed loop system, leading to the $\Htwo$ control problem
%\begin{equation}
%\begin{array}{rl}
%\minimize{\tilde{U}\in\RHinf} & \Htwonorm{X - \M(\tilde{U})}^2 + \rho_u\Htwonorm{\tilde{U}}^2 \\
%\text{s.t.} & \tilde{U}\tilde{P}_{21}^{-1} \in \s,
%\end{array}
%\label{eq:h2_mm}
%\end{equation}
%where $X=C_1(zI-A)^{-1}B_1$ is the state component of the open loop response, and $\M = \frac{1}{z}C_1(zI-A)^{-1}B_2$ is the map from Youla parameter $U$ to the state component of the closed loop response.  In particular, we exploit the orthogonality assumptions \eqref{eq:ortho} imposed on the state space parameters of the generalized plant \eqref{eq:genplant} to separate the state cost $\Htwonorm{X - \M(\tilde{U})}^2$ from the control cost $\rho_u\Htwonorm{\tilde{U}}^2$.
\begin{rem}
A dual argument applies to $\Htwo$ filter design by considering the ``full-control'' setting, cf. \cite{ZDG96} for more details.
\end{rem}
\label{ex:actuators}
\end{example}}

\edit{As illustrated by Example \ref{ex:actuators}, the $\Htwo$ optimal control problem \eqref{eq:the_opt} is simply a more general way of writing the $\Htwo $ state feedback model matching problem -- in Remark \ref{rem:output_feedback} we show how $\Htwo$ output feedback model matching problems can also be put in a similar form.  Writing the $\Htwo$ problem as a linear inverse problem with a least squares like state cost and an explicitly separated control cost already allows us to make connections to classical techniques from statistical inference -- we make further connections in the sequel once suitable convex penalty functions are introduced.}  In order to keep the discussion as streamlined as possible, we make these connections in the context of the Basic LQR problem presented in Example \ref{ex:bLQR}.

\subsubsection{$\rho=0$}  In an inferential context, this is simply ordinary least squares, and is commonly used when $U_*$ is not known \emph{a priori} to have any structure.  Further, the resulting estimate of $U_*$ is unbiased, but often suffers from high error variance.  Moving now to a control context, It is easy to see that this setting corresponds to ``cheap control'' LQR, in which there is no cost on $u_t$ -- under suitable \edit{controllability and observability} assumptions, the resulting state trajectory is deadbeat, but the optimal control law is not necessarily unique.


\subsubsection{$\rho >0$}  \note{This corresponds to Ridge Regression or Tikhonov Regularization \cite{Ridge}.  In an inferential context, this regularizer has the effect of \emph{shrinking} estimates towards 0 -- this introduces bias into the estimator, but reduces its variance, and is often a favorable tradeoff from a statistical perspective.  From a linear algebraic perspective, this is a commonly used technique to improve the numerical conditioning of an inverse problem.  Once again, the interpretation in RFD is clear: this corresponds to standard LQR control with $R = \rho I$; the parameter $\rho$ allows for a tradeoff between control effort and state deviation.  The optimal control action is then {unique} and the resulting state trajectory is generally not deadbeat.}

\subsection{The $\Htwo$ RFD Optimization Problem with an Atomic Norm Penalty}
\label{sec:atoms}
Recall that our strategy for designing controller architectures is to augment the traditional model matching problem \eqref{eq:gen_mm} with a structure inducing penalty, resulting in the RFD optimization problem \eqref{eq:rfd_opt}.  In light of the discussion of the previous subsection, we further specialize the RFD optimization problem to have an $\Htwo$ performance metric and an atomic norm penalty $\norm{\cdot}_\A$.

\begin{defn}
Let $U, \, Y \in \RHinf$ and $\M:\RHinf \to \RHinf$ be of compatible dimension.  The optimization problem
\begin{equation}
\begin{array}{rl}
\minimize{U\in \RHinf} & \Htwonorm{Y - \M(U)}^2+\rho\Htwonorm{U}^2+2\lambda\left\|U\right\|_{\A}\\
\text{s.t.} & U \in \s
\end{array}
\label{eq:h2_opt}
\end{equation}
is called the $\Htwo$ \emph{RFD optimization problem} with parameters $(\rho,\lambda)$, distributed constraint $\s$, and atomic norm penalty $\left\|\cdot\right\|_{\A}$.
\end{defn}

There are two components of note in this definition.  The first is that $\rho$ need not be equal to $\rho_u$, the control cost parameter of the original non-penalized control problem \eqref{eq:the_opt} -- the reasons why a different choice of $\rho$ may be desirable are explained in Section \ref{sec:recovery}.  

The second is the use of an atomic norm penalty function to induce structure.  Indeed, if one seeks a solution $U_*$ that can be composed as a linear combination of a small number of ``atoms'' $\A$, then a useful approach, as described in \ellcitations, \nuccitations, \cite{CRPW12}, to induce such structure in the solution of an inverse problem is to employ a convex penalty function that is given by the atomic norm induced by the atoms $\A$ \approxcitations. Examples of the types of structured solutions one may desire in linear inverse problems include sparse, group sparse and signed vectors,  and low-rank, permutation and orthogonal matrices (see \cite{CRPW12} for a more extensive list).

Specifically, if one assumes
that
\begin{equation}
U=\sum_{i=1}^{r}c_{i}A_{i},\ A_{i}\in\A,\ c_{i}\geq0
\label{eq:decomp}
\end{equation}
for a set of appropriately scaled and centered atoms $\A$,
and a small number $r$ relative to the ambient dimension, then solving
\begin{equation}
\begin{array}{rl}
\underset{U}{\mathrm{minimize}}  &  \cost{U;Y,\M} + 2\lambda\|U\|_\A
\end{array}
\end{equation}
with the atomic norm $\|\cdot\|_\A$ given by the gauge function\footnote{If no {such $t$ exists}, then $\|X\|_\A = \infty$.} 
\begin{equation}
\begin{array}{rcl}
||U||_{\A}: & = & \inf\{t\geq0\, \big{|}\, U\in t\mathrm{conv}(\A)\}\\
 & = & \inf\{\sum_{A\in\A}c_{A}\, \big{|}\, U=\sum_{A\in\A}c_{A}A,\, c_A \geq 0\}
\end{array}
\label{eqn:atomnorm}
\end{equation}
results in solutions that are both consistent with the data as measured in terms of the cost function $\cost{\cdot;Y,\Cl}$, and that are sparse in terms of their atomic descriptions, i.e., are a nonnegative combination of a small number of elements from $\A$.  \edit{Note that the unit ball of the atomic norm is given by the convex hull of its constituent atoms -- as such, atomic norms are convex functions.}

%The geometric justification behind the success of these methods is
%that the unit-ball of an atomic norm is appropriately ``pointy'' in high dimensions,
%and thus solutions are likely to lie on lower dimensional faces of the norm-ball, inducing the desired simple structure.

%\subsection{RFD Atomic Norms}
%With these optimizations defined, we now present a catalog of atomic norms that are useful in the context of RFD -- in particular,

Our discussion in $\S$\ref{sec:RFDQI} on designing controller architecture by finding structured solutions to the model matching problem \eqref{eq:gen_mm} suggests natural atomic sets for constructing suitable penalty functions for RFD.  We make this point precise by showing that actuator, sensor, and/or communication delay design can all be performed through the use of a purposefully constructed atomic norm. 
 We introduce several novel penalty functions for controller architecture design, most notably for the simultaneous design of actuator, sensor and communication delays.   Further, all regularizers that have been considered for control architecture design in the literature (cf. \cite{LFJ13,JRM14,DLFM12,XB07,FLJ13,MC_CDC14,DJL14,M_CDC13_codesign, M_TCNS14}, among others) may be viewed as special instances of the atomic norms described below.

%Suppose that $U \in \RHinf^{n_a \times n_s}$  is a map from sensor measurements to actuator commands -- this is true, for example, when $U$ is the Youla Parameter in a model matching problem, or when $U$ is a static state or output feedback gain.  Then each non-zero row of $U(z)$ corresponds to an actuator that the controller uses, and likewise, each non-zero column corresponds to a sensor that the controller uses.  Further sparsity patterns present within rows/columns of the power series elements $U_t$ of $U(z)$ can be interpreted as information exchange constraints imposed by an underlying communication network between the sensors and actuators.
%
%We use these observations to define atomic norms that induce simple controller architectures.
In what follows, the atomic sets that we define are of the form
\begin{equation}
\A = \displaystyle \bigcup_{\Aa \in \mathscr{M}} \Aa \cap k_{\Aa} \mathcal{B}_{\Htwo},
\label{eq:asets}
\end{equation}
for $\mathscr{M}$ an appropriate set of subspaces, $\{k_{\Aa}\}$ a set of normalization constants indexed by the subspaces $\Aa \in \m$, and $\mathcal{B}_{\Htwo}$ the $\Htwo$ unit norm ball; see the concrete examples below.  %In order to make explicit that the subspaces in $\m$ are associated with a specific atomic set $\A$ we use the same subscript label for both the atomic set and the set of subspaces, e.g., $\A_\text{act}$ is defined in terms of the collection of subspaces $\m_\text{act}$.
Note that we normalize our atoms relative to the $\Htwo$ norm as this norm is isotropic; hence this normalization ensures that no atom is preferred over another within a given family of atoms $\A$.  We use $n_s$ and $n_a$ to denote the total number of sensors and actuators, respectively, that are available for the RFD task.

\subsubsection{Actuator Norm} \note{We choose the atomic set to be transfer functions in $\RHinf^{n_a \times n_s}$ that have exactly one non-zero row with unit $\Htwo$ norm, i.e., suitably normalized Youla parameters that use only one actuator.  Specifically, the set of subspaces \eqref{eq:asets} in this context is
\begin{equation}
\m_{\text{act}} := \left\{ \Aa \subset \RHinf^{n_a \times n_s} \, \big{|} \, \text{$\Aa$ has one nonzero row} \right\},
\label{eq:act_sub}
\end{equation}
 leading to the atomic set
\begin{equation}
\A_{\text{act}} := \left\{ e_i V \, \big{|} \, V \in \RHinf^{1 \times n_s},\, \Htwonorm{V} = 1\right\}.
\label{eq:act_atoms}
\end{equation}
The resulting \emph{Actuator Norm} is then given by
\begin{equation}
\norm{U}_{\text{act}} = \sum_{i=1}^{n_a} \Htwonorm{e_i^\top U},
\label{eq:act_norm}
\end{equation}
which is akin to a Group Lasso penalty \cite{GroupLasso}.  In particular, each ``group'' corresponds to a row of the Youla parameter.}

\subsubsection{Sensor Norm}  Similar to the previous case, we choose the atomic set to be transfer functions in $\RHinf^{n_a \times n_s}$ that have exactly one non-zero column with unit $\Htwo$ norm, i.e., suitably normalized Youla parameters that use only one sensor.  Specifically, the set of atoms
\begin{equation}
\A_{\text{sns}} := \left\{ We_i^\top \, \big{|} \, W \in \RHinf^{n_a \times 1},\, \Htwonorm{W} = 1\right\}
\label{eq:sns_atoms}
\end{equation}
leads to the \emph{Sensor Norm}
\begin{equation}
\norm{U}_{\text{sns}} = \sum_{i=1}^{n_s} \Htwonorm{Ue_i},
\label{eq:sns_norm}
\end{equation}
which is also akin to a Group Lasso penalty \cite{GroupLasso}.

%\paragraph{Joint Actuator/Sensor Norm} Here the atomic set is naturally taken to be the union of $\mathcal{A}_{\text{act}}$ and $\mathcal{A}_{\text{sns}}$, i.e.
%\begin{equation}
%\mathcal{A}_{\text{joint}} :=  \mathcal{A}_{\text{act}} \cup \mathcal{A}_{\text{sns}},
%\label{eq:joint_atoms}
%\end{equation}
%and leads to the Joint Norm
%\begin{equation}
%\begin{array}{rl}\norm{U}_{\text{joint}} = \min_{V_i,\, W_j} & \sum_{i=1}^{n_u} \Htwonorm{V_i} + \sum_{j=1}^{n_y} \Htwonorm{W_j}  \\
%\text{s.t.} & U = \sum_{i=1}^{n_u} e_i V_i + \sum_{j=1}^{n_y} W_j e_j^\top.
%\end{array}
%\label{eq:joint_norm}
%\end{equation}

\subsubsection{Communication Link Norm}
% We begin with the simple case of $U$ corresponding to a static feedback gain.  In this case, each non-zero element $U_{ij}$ can be interpreted as a direct communication link from sensor $j$ to actuator $i$.  If no additional constraints or structure are imposed, then the appropriate set of atoms is
%\begin{equation}
%\A_{\text{static}} := \left\{ E_{ij} \right\},
%\label{eq:static_atoms}
%\end{equation}
%which leads to the familiar $\ell_1$-norm:
%\begin{equation}
%\norm{U}_{\text{static}} = \sum_{i=1}^{n_a} \sum_{j=1}^{n_s}\left|U_{ij}\right|.
%\label{eq:static_norm}
%\end{equation}
\note{As described in \S\ref{sec:RFDQI}, the communication design task is: given an existing communication graph, to select which additional links to introduce into the existing communication graph.  An atom in $\A_{\text{comm}}$ corresponds to such an additional link.  We provide an example of such an atomic set for a simple system, and refer the reader to \cite{M_TCNS14} for a more general construction.  
\begin{figure}[!h]
\centering
\includegraphics[width = .15\textwidth]{3chain}
\caption{Three player chain system}
\label{fig:4chain}
\end{figure}
In particular, consider a three player chain system, with physical topology illustrated in Figure \ref{fig:4chain}, such that $P_{22}$ lies in the subspace
\[
\s:= \frac{1}{z}\begin{bmatrix} \ast & 0 & 0  \\ 0 & \ast & 0 \\ 0 & 0 & \ast \end{bmatrix} \oplus 
\frac{1}{z^2}\begin{bmatrix} \ast & \ast & 0  \\  \ast & \ast & \ast \\ 0 & \ast & \ast \end{bmatrix} \oplus 
\frac{1}{z^3}\Rp,
\]
where $\ast$ is used to denote $\R$ to reduce notational clutter.
We consider an existing communication graph matching the physical topology illustrated in Figure \ref{fig:4chain} so that the induced distributed subspace constraint, as described in \S\ref{sec:RFDQI}, is given precisely by $\s$.  It can be checked that $\s$ is then QI with respect to $P_{22}$.  We consider choosing from two additional links to augment the communication graph: a directed link from node 1 to node 3, and a directed link from node 3 to node 1.  Then $\m_{\text{comm}} = \{\Aa_{13} , \Aa_{31} $\}, where its component subspaces are given by
\begin{equation*}
\begin{array}{rclrcl}
\Aa_{13} &=& \frac{1}{z^2}\begin{bmatrix} 0 & 0 & 0  \\  0 & 0 & 0 \\ \ast & 0 & 0 \end{bmatrix}, 
\Aa_{31} &=& \frac{1}{z^2}\begin{bmatrix} 0 & 0 & \ast  \\  0 & 0 & 0 \\ 0 & 0 & 0 \end{bmatrix}.
\end{array}
\end{equation*}
In particular, each subspace $\Aa_{ij}$ corresponds to the additional information available to the controller \emph{uniquely} due to the added link from sensor $j$ to actuator $i$.
The resulting \emph{Communication Link Norm} $\norm{\cdot}_{\text{comm}}$ is then constructed according to \eqref{eq:asets} with all normalization constants $k_{\Aa}=1$.
%To streamline presentation and avoid introducing additional notation, we assume that $n_s = n_a$ so that $U(z)$ is square.  Then, given a communication graph between sensors and actuators with adjacency matrix $\Gamma$,  each power series element of $U^{(t)}$ satisfies $\supp{U^{(t)}}\subseteq \supp{\Gamma^{t-1}}$ under mild conditions (cf. \cite{M_TCNS14}) -- the interpretation of the support nesting condition is that the delay from sensor $j$ to actuator $i$ is given by the length of the shortest path from node $j$ to node $i$ in the graph $\Gamma$.  
We note that it is akin to the latent Group Lasso\footnote{This was formerly referred to as the Group Lasso with Overlap \cite{JOV09}.} \cite{OJV11}.
}%Each nonzero atom in the resulting decomposition is conceptually equivalent to adding a small number of additional links to the original simple communication graph that guarantees that QI holds. %Note that we abuse notation and let $\Aa \in \A_{\text{den}}$ denote subspaces defined by the support of a single generic atom.

  %Further, the static case \eqref{eq:static_norm} is a special case of this norm, in which each atom $U_a$ satisfies $\left|\supp{U_a}\right|=1$.

\subsubsection{Joint Actuator and Sensor Norm}  Conceptually, each atom corresponds to a controller that uses only a small subset of actuators and sensors. As each row of the Youla parameter $U$ corresponds to an actuator and each column to a sensor, the atomic transfer matrices have support defined by a submatrix of $U(z)$.  Specifically, we choose atoms with at most $k_a$ actuators and $k_s$ sensors:
\begin{multline}
\m_{\text{act+sns}} := \left\{ \Aa \subset \RHinf^{n_s\times n_a} \, \big{|} \, \supp{\Aa} \text{is a submatrix} \right. \\ \left. \text{with at most $k_a$ nonzero rows}  \text{ and $k_s$ nonzero columns} \right\}
%\A_{\text{act+sns}} := \bigcup_{\Aa \in \m_{\text{act+sns}}} \Aa \cap \left(\text{card}(\Aa)+.1\right)^{-\frac{1}{2}} \mathcal{B}_{\Htwo}
%\left\{ V_{\mathcal{M}}\, \big{|} \, \mathcal{M} \in \mathscr{M}, \Htwonorm{V_\mathcal{M}} = \left(\text{card}(\mathcal{M})+.1\right)^{-\frac{1}{2}}\right\},
\label{eq:act+sns_atoms}
\end{multline}
The scaling terms $k_{\Aa}$ in the definition of the atomic set \eqref{eq:asets} are given by $k_{\Aa}= \left(\text{card}(\Aa)+.1\right)^{-\frac{1}{2}}$, and are necessary as some of the atoms are nested within others -- the additional $.1$ can be any positive constant, and controls how much an atom of larger cardinality is preferred over several atoms of lower cardinality.
The resulting \emph{Actuator+Sensor Norm} is then constructed according to \eqref{eq:asets} and
%\begin{equation}
%\begin{array}{rl}
%\norm{U}_{\text{act+sns}} = \displaystyle \min_{\{U_i\} }& \displaystyle \sum_{i = 1}^{ |\m_{\text{act+sns}}|} \left(\text{card}(\Aa_i)+.1\right)^{\frac{1}{2}} \Htwonorm{U_i} \\
%\text{s.t.} & U = \displaystyle \sum_{i = 1}^{ |\m_{\text{act+sns}}|}{U_i}, \\
%& U_i \in \Aa_i, \,\text{for $i=1,\dots,|\m_{\text{act+sns}}|$},
%\end{array}
%\end{equation}
%which
 is also akin to the latent Group Lasso \cite{OJV11}.

\subsubsection{Joint Actuator (and/or Sensor) and Communication Link Norm}
%We begin again with the simpler case of when $U$ is a static feedback gain.  In this case, this problem can be viewed as simultaneously inducing sparsity at the actuator (row) level, and inducing sparsity \emph{within} each row.  The appropriate regularizer can be viewed as a nesting of atomic norms: one atomic norm defined by \eqref{eq:act_atoms} being applied to $U$, and further, another atomic norm defined by \eqref{eq:static_atoms} being applied to each atomic element $U_a, a \in \mathcal{A}$.  It can be checked that the  resulting penalty is then given by
%\begin{equation}
%\norm{U}_{\text{act+static}} = (1-b)\norm{U}_{\text{static}} + b\norm{U}_{\text{act}},
%\end{equation}
%for some constant $b \in [0,1]$.  The first term of this penalty induces sparsity \emph{within} rows, while the second induces sparsity at the row level.  This is a special case of the Sparse Group LASSO penalty \cite{SFHt13}.

This penalty can be viewed as simultaneously inducing sparsity at the communication link level, while further inducing row sparsity as well.  The general strategy is to combine the actuator and communication link penalties in a convex manner.  We suggest two such approaches, one based on taking their weighted sums and the other based on taking their ``weighted maximum.''  In particular, we define the joint actuator \emph{plus} communication link penalty to be:
\begin{equation}
\norm{U}_{\text{act+comm}} = (1-\theta)\norm{U}_{\text{comm}} + \theta\norm{U}_{\text{act}},
\end{equation}
for some $\theta\in [0,1]$,
and the \emph{max} actuator/communication link penalty to be
\begin{equation}
\norm{U}_{\max\{\text{act},\text{comm}\}} = \max\left\{(1-\theta)\norm{U}_{\text{comm}}, \theta\norm{U}_{\text{act}}\right\},
\end{equation}
for some $\theta \in [0,1]$.
The analogous Sensor and Communication Link penalties, as well as Sensor+Actuator and Communication link penalties can be derived by replacing $\A_{\text{act}}$ with either $\A_{\text{sns}}$ or $\A_{\text{act+sns}}$.

%As we will show shortly, this simple definition encompasses an extremely broad range of RFD problems.  Before proceeding however, we specialize this general optimization to a particularly important case, namely that where the performance criteria is taken to be the $\Htwo$ norm of the closed loop system, and where the penalty is taken to be an atomic norm.

%In this definition, we explicitly separate out the ``state-cost'' $\Htwonorm{Y + \M(U)}^2$ from the ``control cost'' $\rho\Htwonorm{U}^2$ of the closed loop response -- doing so allows us to connect the $\Htwo$ {RFD optimization} to several well established methods from SLIP, as described in the next subsection.
%
%We begin with a simple illustrative example of how a standard control problem can be mapped into a $\Htwo$ {RFD optimization}, before introducing a problem that we study in much greater detail in Section \ref{sec:recovery}.
%
%\begin{example}[Basic LQR]
%Consider the basic LQR problem given by
%\begin{equation}
%\begin{array}{rl}
%\minimize{u\in \ell_2} & \sum_{t=0}^\infty \|Cx_t\|_{\ell_2}^2 + \|Du_t\|_{\ell_2}^2 \\
%\text{s.t.} & x_{t+1} = Ax_t + Bu_t,\ x_0 = \xi,
%\end{array}
%\end{equation}
%and assume that $D^\top D = \rho I$, for some $\rho>0$.
%
%Define $Y^{(t)} = CA^{t}\xi$ for $t\geq 0$, $U^{(t)} = u_t$, and $\M(U) = H\ast U$, where $H\in \ell_{2,e}$ with $H^{(0)}=0$, and $H^{(t)} = CA^{t-1}B$ for $t\geq 1$.  We can then rewrite the basic LQR problem as
%\begin{equation}
%\begin{array}{rl}
%\minimize{U\in \RHinf} & \Htwonorm{Y+\M(U)}^2 + \rho\Htwonorm{U}^2.
%\end{array}
%\label{eq:noreg}
%\end{equation}
%\label{ex:bLQR}
%Adding an appropriate penalty, such as the Actuator Norm, then converts this problem into one of the form \eqref{eq:the_opt}.
%\end{example}
%

\subsection{Further Connections with Structured Inference}
%Before proceeding with the technical development, we make further connections between the $\Htwo$ RFD optimization \eqref{eq:h2_opt} with atomic norm penalty and the structured inference literature.  
As already noted in \S\ref{sec:cost_fcns}, by choosing different values of $\rho$ for $\lambda=0$ we are able to recover control-theoretic analogs to Ordinary Least Squares and Ridge Regression \cite{Ridge}.  Noting that the actuator norm penalty \eqref{eq:act_norm} is akin to the Group Lasso \cite{GroupLasso}, we now discuss how control theoretic analogs of the Group Lasso and Group Elastic Net \cite{ElasticNet}  can be obtained by setting $\lambda >0$ in \eqref{eq:h2_opt} and using the Actuator Norm \eqref{eq:act_norm} penalty.    To simplify the discussion, we once again consider these connections in the context of the basic LQR problem introduced in Example \ref{ex:bLQR}, now augmented with the actuator norm penalty \eqref{eq:act_norm}.

%\begin{table*}[!t]
%\centering
%\begin{tabularx}{\textwidth}{|X|XXX|XXX|}
%\hline
% 			Parameters		& SLIP Problem & SLIP Structure & SLIP Tradeoff &  RFD Problem & {RFD~Structure} & RFD Tradeoff  \\ \hline
% $\lambda = 0$, $\rho=0$ &Ordinary \newline Least Squares & None & N/A & Cheap Control \newline LQR & Deadbeat response & N/A   \\ \hline
% $\lambda = 0$, $\rho>0$ &Ridge Regression & Small Euclidean norm  & Bias, Variance & LQR & Small control action& State deviation,\newline Control effort \\ \hline
% $\lambda > 0$, $\rho=0$ & Group LASSO & Group sparsity & Bias, Variance, \newline Model complexity & RFD LQR &  Sparse actuation & State deviation,\newline Control effort,\newline Actuation complexity \\ \hline
%  $\lambda > 0$, $\rho>0$ & Group Elastic Net & Correlated \newline group sparsity & Bias, Variance, \newline Model complexity & RFD LQR & Correlated \newline sparse actuation & State deviation,\newline Control effort, \newline Actuation complexity \\ \hline
%\end{tabularx}
%\caption{A dictionary relating various SLIP problems in statistical inference and Actuator RFD problems.}
%\label{tab:dict}
%\end{table*}


%\paragraph{$\lambda >0$, $\rho=0$} In SLI, this corresponds to Group LASSO regression, and is commonly used in the $n \ll p$ regime when $U^*$ is known \apriori to be group sparse.  When the groups correspond to single elements, this becomes LASSO regression, in which a sparse model is estimated.  It has been shown that the Group LASSO estimator can produce consistent estimates (with high probability) if $S$ satisfies certain incoherence assumptions (akin to the restricted isometry property \cite{CT05}) despite apparent ill-posedness of the inference problem.  Once again, this regularizer has the effect of \emph{shrinking} estimates toward 0, introducing an increase in bias in favor of a decrease in variance.  Further, the Group LASSO estimator performs the additional task of \emph{group selection} -- that is to say it induces sparsity at the group level, helping in the interpretability of the resulting model.
%
%In RFD, we find ourselves in a non-standard control setting, in which the control effort penalty both induces shrinkage and group sparsity -- that is to say both the magnitude of the control signal and the \emph{number of actuators used} decrease as $\lambda$ increases. %Carrying over the interpretation from SLI suggests that this variant of RFD is well suited for controller design when the system is \emph{over-actuated}, that is to say when $n_y \ll n_u$.  This implication will be further explored in the following sections.

\note{
In structured inference problems, the setting $\lambda>0,\, \rho >0$ corresponds to Group Elastic-Net regression.  If the groups are single elements, this becomes the traditional Elastic Net and Lasso.  The singleton group setting with $\lambda>0$, $\rho = 0$ corresponds to Lasso regression, and this inference method is employed when the underlying model is known to be sparse -- in particular, the Lasso penalty is used to select which elements $U^*_i$ of the model are non-zero \ellcitations.  Continuing with the singleton group setting, if both $\lambda>0$ and $\rho>0$, then the corresponding inferential approach is called the Elastic Net.  In addition to the sparsity-inducing properties of the Lasso, the Elastic Net also encourages automatic clustering of the elements \cite{ElasticNet} -- in particular, $\rho>0$ encourages the simultaneous selection of highly correlated elements (two elements $U^*_i$ and $U^*_j$ are said to be highly correlated if $\Cl(U^*_i) \approx \Cl(U^*_j)$). Thus $\rho$ can be seen as a parameter that can be adjusted to leverage a prior of \emph{correlation} in the underlying measurement operator $\M$.  These interpretations carry over to more general groups in a natural way.%It has been shown that the Group LASSO estimator can produce consistent estimates (with high probability) if $S$ satisfies certain incoherence assumptions (akin to the restricted isometry property \cite{CT05}) despite apparent ill-posedness of the inference problem.
}

In RFD, this setting corresponds to our motivating Example \ref{ex:bLQR} augmented with the actuator norm penalty, in which we design the controller's actuation architecture.  As each atom corresponds to an actuator, this RFD procedure then selects a small number of actuators.  Porting the clustering effect interpretation from the structured inference setting, we see that $\rho$ promotes the selection of actuators that have similar effects on the closed loop response.  In particular, this suggests that for systems in which no such similarities are expected, $\rho$ should be chosen to be small (or 0) during the RFD process, even if the original LQR problem had non-zero control cost.




==> rfd_as_struct2.tex <==
Traditional controller synthesis methods within the framework of \emph{model matching} can be framed as optimizations of the form\footnote{Exactly how this can be done, as well as how to accommodate \emph{quadratically invariant} distributed constraints, will be shown in \S \ref{sec:model_match}.}
\begin{equation}
\begin{array}{rl}
\minimize{U\in \RHinf} & \cost{Y + \M(U)}\\
\end{array}
\label{eq:trad_opt}
\end{equation}
for $Y$ the open loop response of the system, $U$ the Youla parameter, $\M$ the map from the controller to the closed loop response, and $\cost{\cdot}$ the performance metric being optimized, such as the $\Htwo$ or $\Hinf$ norm.

Our goal is to modify such synthesis methods to co-design both the controller architecture, as well as the traditional control laws themselves.  We re-iterate that by
the \emph{architecture} of a controller, we mean the actuators, sensors, and communication links between them.  Within this framework, we show that designing the controller architecture is equivalent to designing suitably \emph{structured} Youla parameters $U$.

In particular, if we view $U$ as a map from all potential sensors to all potential actuators, using all possible communication links between these actuators and sensors, the architectural design task is that of selecting which actuators, sensors and communication links need to be used to achieve a certain performance level.  This task is naturally viewed as trying to find a \emph{structured approximation} of the optimal centralized controller that maximally utilizes the available architectural choices.  In order to compute such an approximation, we modify the problem \eqref{eq:trad_opt} by augmenting it with a penalty function, or regularizer, to induce structure in the controller which has a direct interpretation in terms of the resulting \emph{architecture} of the control system.  In other words, we seek an ``architecturally sparse'' approximation of a hypothetical optimal controller that maximally utilizes the available architectural resources.  

\begin{defn}
Let $U\in \RHinf$, $Y\in\eltwoe$, and $\M:\RHinf \to \eltwoe$ be of compatible dimension.  The optimization
\begin{equation}
\begin{array}{rl}
\minimize{U\in \RHinf} & \cost{Y + \M(U)}+2\lambda\Omega\left(U\right)
\end{array}
\label{eq:rfd_opt}
\end{equation}
is called a \emph{RFD optimization} with performance metric $\cost{\cdot}$, and penalty $\Omega\left(\cdot\right)$.
\end{defn}

Temporarily ignoring computational considerations, we catalog the various types of penalty functions $\Omega\left(\cdot\right)$ that are useful for RFD.  In particular, notice that each non-zero row of $U(z)$ corresponds to an actuator that the controller uses, and likewise, each non-zero column corresponds to a sensor that the controller uses.  Further sparsity patterns present within rows/columns of the power series elements $U^{(t)}$ of $U(z)$ can be interpreted as information exchange constraints imposed by an underlying communication network between the sensors and actuators.  With these observations, it becomes clear that $\Omega$ should be chosen to be an appropriate structural penalty defined by the RFD task:
\begin{itemize}
\item \textbf{Actuation design}: $\Omega$ should penalize the number of non-zero rows of $U(z)$.
\item \textbf{Sensing design}: $\Omega$ should penalize the number of non-zero columns of $U(z)$.
\item \textbf{Communication design}: $\Omega$ should penalize specific sparsity patterns within the the impulse response of $U(z)$ that correspond to an added communication link.
\item \textbf{Joint design}: $\Omega$ should penalize a weighted sum of either the actuation, sensing or communication penalties, depending on what subset of the architecture is being co-designed.
\end{itemize}

The rest of this section is organized as follows:  we first introduce the model matching framework in \S \ref{sec:model_match} and show how it maps to optimizations of the form \eqref{eq:trad_opt}.  In \S \ref{sec:RFDQI}, we show how \emph{quadratically invariant} distributed constraints can be accommodated, and more importantly that we can perform the architectural design task on the Youla parameter $U$, rather than the original controller.

\subsection{Convex Model Matching}
\label{sec:model_match}

\begin{figure}[h!]
\centering
\includegraphics[width = .2\textwidth]{genplant}
\caption{A diagram of the generalized plant defined in \eqref{eq:genplant}.}
\label{fig:genplant}
\end{figure}
In order to discuss a broad range of RFD optimizations, we introduce the notion of a \emph{generalized plant}, a standard tool in robust and optimal control \cite{ZDG96}.  In particular, consider the system described by
\begin{equation}
P = \begin{bmatrix}
P_{11} & P_{12} \\
P_{21} & P_{22}
\end{bmatrix}
= \left[\begin{array}{c|cc}
A & B_{1} & B_{2} \\ \hline
C_{1} & 0 & D_{12} \\
C_{2} & D_{21} & 0
\end{array}\right]
\label{eq:genplant}
\end{equation}
where $P_{ij} = C_{i}(zI-A)^{-1}B_{j} + D_{ij}$.  As illustrated in Figure \ref{fig:genplant}, this system describes the four transfer matrices from the disturbance and control inputs $w$ and $u$, respectively, to the controlled and measured outputs $y$ and $m$, respectively.  We make the (slightly modified) standard assumptions that $D_{12}\begin{bmatrix} C_1^\top & D_{12}^\top \end{bmatrix} =  \begin{bmatrix} 0 & \rho_u I \end{bmatrix}$, and that $D_{21}^\top\begin{bmatrix} B_1 & D_{21} \end{bmatrix} =  \begin{bmatrix} 0 & \rho_w I \end{bmatrix}$, for some $\rho_u, \rho_w \geq 0$.

It is also convenient to introduce finite horizon variants of these various operators.  Restricted to a finite horizon $n$, causal linear operators are isomorphic to block-lower triangular matrices.  We denote this subspace by $\T:= {\Rp^{\leq n}}$.

In order to reduce the technical overhead required, our discussion focusses on the finite horizon variant of these problems -- as such, we fix a horizon $n$ and overload notation by dropping the $\leq n$ superscript on $P_{ij}^{\leq n}$. We conclude the section with how to extend the discussion to infinite horizon problems through the use of appropriate Youla-Kucera parameterizations.

Letting $u(z) = K(z)m(z)$, for a causal linear controller $K$, a general optimal control problem with convex cost function $\cost{\cdot}$ can then be written as
\begin{equation}
\begin{array}{rl}
\minimize{K\in\T} & \cost{P_{11} - P_{12}K(I-P_{22}K)^{-1}P_{21}} \\
\text{s.t.} & K \in \s,
\end{array}
\label{eq:gen_opt}
\end{equation}
 where the expression in the cost function corresponds to the closed loop map from $w$ to $y$.

When the additional distributed constraint that $K\in\s$ is not present, a standard and general approach to solving such a problem is to first convert it into a \emph{convex model matching problem} through the change of variables $U:= K(I-P_{22}K)^{-1}$; the optimal $K$ can then be recovered via $K = (I+UP_{22})^{-1}U$.  As lower block triangular matrices form an \emph{algebra}, it is easily verified that both $K$ and $U$ are in $\T$, i.e. causality is preserved under the above change of variables.

However, when such a distributed constraint $\s$ is present, it is known that a necessary and sufficient condition for such a constraint to be invariant under such a change of variables is that it be \emph{quadratically invariant} with respect to $P_{22}$ \cite{RL06,LL11_QI}.

\begin{defn}[Quadratic Invariance]
A subspace $\s$ is \emph{quadratically invariant} (QI) with respect to $P_{22}$ if $KP_{22}K \in \s \ \forall K \in \s$.
\label{def:QI}
\end{defn}

In particular, when QI holds, we have that $K \in \s$ if and only if $K(I-P_{22}K)^{-1} \in \s$, allowing us to convert the general optimal control problem \eqref{eq:gen_opt} to the following convex model matching problem

\begin{equation}
\begin{array}{rl}
\minimize{U\in\T} & \cost{P_{11} - P_{12}UP_{21}}\\
\text{s.t.} & U \in \s.
\end{array}
\label{eq:gen_mm}
\end{equation}
By adding a RFD atomic norm penalty to optimization \eqref{eq:gen_mm}, we obtain a RFD optimization \eqref{eq:rfd_opt}.  In particular, we have that $Y := P_{11}$ and $\M(U) := P_{12}UP_{21}$.

This framework is sufficiently general as it allows for a unified treatment of all structured optimal control problems in which the optimal structured controller is known to be linear, and can be computed via convex optimization \cite{RL06,LL11_QI}.  These include state and output feedback problems in either centralized or QI distributed settings.

\subsubsection{Static or Dynamic}
With the exception of the centralized state-feedback setting, it is known that the optimal controller is dynamic, and therefore restricting our analysis to dynamic controllers is natural.  In the centralized setting, given the equivalence between static and dynamic state-feedback, once an appropriate actuation architecture\footnote{For a system to be centralized, there can be no communication constraints, and for it to be state-feedback, there can be no sensing constraints, leaving only actuation architecture design as a possible RFD task.} is identified via a RFD optimization, traditional methods can then be used to solve for a static state-feedback controller restricted to that architecture.  Further as we will show in Section \ref{sec:recovery}, the RFD optimization approach is amenable to analysis guaranteeing \emph{optimal structure recovery}.

\subsubsection{Extensions to Infinite Horizon}
Although the details are beyond the scope of this paper, the above discussion extends to infinite horizon problems as well -- when the open-loop plant is stable, the general approach described applies, with $U=K(I-P_{22}K)^{-1}$ now becoming the Youla parameter of the problem.  In the case of unstable plants, an appropriate \emph{structure preserving} Youla-Kucera parameterization must be employed, cf.  \cite{SM12,LD14} for examples of such parameterizations, and \cite{M_TCNS14} for an example of RFD using such a parameterization.


\subsection{Quadratically Invariant Architectures}
\label{sec:RFDQI}
As the structural co-design task is performed in the $U$ domain, care must be taken to ensure that this structure is preserved under the change of variables.  As elements in $\T$ form an algebra, we focus on ensuring that any additional structure imposed on $U$ is preserved in $K$.  In particular, RFD can be viewed as designing a subspace $\D$ in which $U$ lies: only if $\s\cap\D$ is QI under $P_{22}$ can we guarantee that $K =  (I+UP_{22})^{-1}U \in \s\cap\D$ as well.

\paragraph{Actuator Design}
For actuator design, notice that the resulting subspace $\D_{\text{act}}$ is defined by its row-sparsity: in particular, the $i^{\text{th}}$ row of $U$ is non-zero if and only if the corresponding actuator was selected by the RFD optimization.  More precisely, $K\in\D_{\text{act}}$ if and only if the row support of $K$ is a subset of that of $\D_{\text{act}}$.  It is easily verified that if $K \in \D_{\text{act}}$, then right multiplication leaves $\D_{\text{act}}$ invariant, i.e. $KX \in \D_{\text{act}}$ for all compatible $X$. It then follows from Definition \ref{def:QI} that $\D_{\text{act}}$ is QI under any plant $P_{22}$.  It follows from the results\footnote{In particular, since removing actuators does not change the communication delays between the remaining actuators and sensors, if the delay based conditions in \cite{RCL10}  hold when all actuators are present, they also hold with any subset of them being present.} in \cite{RCL10} that $\D \cap \s$ is QI under any $P_{22}$ for which $\s$ is QI.

\paragraph{Sensor and Joint Actuator/Sensor Design}
A similar argument applies to sensor placement, where $\D_{\text{sns}}$ is now defined by column-sparsity, and we have that left multiplication leaves $\D_{\text{sns}}$ invariant.  Joint actuator/sensor placement also satisfies the QI property for all plants $P_{22}$; to see this, note that $\D_{\text{sns}+{\text{act}}}$ is defined in terms of both row and column-sparsity.  By virtue of the previous discussion, it follows that $KP_{22}K \in \D_{\text{sns}+{\text{act}}}$ for any $K \in\D_{\text{sns}+{\text{act}}}$, as left multiplication leaves column-sparsity invariant, whereas right multiplication leaves row-sparsity invariant.

\paragraph{Communication and Joint Communication/Actuator/Sensor Design}
Designing communication constraints is a more involved task, the details of which are beyond the scope of this paper.  However, we note that it is possible to construct  penalties (cf. \cite{M_TCNS14} for an example) such that the resulting constraint set $\D_{\text{dyn}}$ is QI, and that by the results of \cite{RCL10} and the previous discussion, combining communication constraint design with actuator/sensor design still leads to QI constraint sets.

Thus, for all of the co-design problems relevant to \emph{architecture} design, the RFD task can be performed via a model matching problem.

\begin{example}
Suppose that different RFD optimizations are performed on a system with three possible actuators and three possible sensors, resulting in the various sparsity patterns in $U(z)$ shown on the far right of Figure \ref{fig:patterns}.  It is easily seen by inspection that the resulting sparsity patterns are QI. In particular Figures \ref{fig:patterns} a) through c) correspond to centralized RFD optimizations (this can be seen from the full matrices in the center of the LHS), and d) to a RFD optimization subject to lower triangular constraints, a special case of a nested information constraint\footnote{Nested information constraints are a well studied class of QI distributed constraints, cf. \cite{LL11, S13, SP10, TP14} for examples.}.

\begin{figure}[h!]
\centering
\includegraphics[width = .45\textwidth]{patterns}
\caption{Examples of QI sparsity patterns generated via a) actuator, b) sensor, and c) actuator/sensor RFD procedures without any distributed constraints, and d) of a QI sparsity pattern generated via actuator RFD subject to nested information constraints.}
\label{fig:patterns}
\end{figure}
\end{example}



==> rfd_as_struct3.tex <==
\note{Under standard assumptions  \cite{ZDG96},} traditional controller synthesis methods within the framework of \emph{model matching} can be framed as linear inverse problems of the form
\begin{equation}
\begin{array}{rl}
\minimize{U\in \RHinf} & \cost{U;Y,\Cl}\\
\end{array}
\label{eq:trad_opt}
\end{equation}
where $Y$ is the open loop response of the system, $U$ is the Youla parameter, $\Cl$ is \note{a suitably defined} linear map from the Youla parameter $U$ to the closed loop response, and $\cost{\cdot;Y,\Cl}$ is a performance metric \edit{that measures the size of the closed loop response (i.e., the size of the deviation between $Y$ and $\Cl(U)$), such as the $\Htwo$ or $\Hinf$ norm.}  

We make this connection clear in the following subsection and we \edit{also recall how} to incorporate \emph{quadratically invariant} \cite{RL06} distributed constraints on the controller into this framework.  
\edit{
\begin{rem}
We use this non-standard notation to facilitate comparisons with the structured inference literature.  In particular, this notation emphasizes that the optimal linear controller synthesis task can be viewed as one of solving a linear inverse problem with ``data'' specified by the open loop response $Y$ of the system and the map $\Cl$ from the Youla parameter to the closed loop response.
\end{rem}}

\subsection{Convex Model Matching}
\label{sec:model_match}

\begin{figure}[h!]
\centering
\includegraphics[width = .2\textwidth]{genplant}
\caption{A diagram of the generalized plant defined in \eqref{eq:genplant}.}
\label{fig:genplant}
\end{figure}
In order to discuss a broad range of model matching problems, we introduce the \emph{generalized plant}, a standard tool in robust and optimal control \cite{ZDG96}.  In particular, consider the system described by
\begin{equation}
P = \begin{bmatrix}
P_{11} & P_{12} \\
P_{21} & P_{22}
\end{bmatrix}
= \left[\begin{array}{c|cc}
A & B_{1} & B_{2} \\ \hline
C_{1} & 0 & D_{12} \\
C_{2} & D_{21} & 0
\end{array}\right]
\label{eq:genplant}
\end{equation}
where $P_{ij} = C_{i}(zI-A)^{-1}B_{j} + D_{ij}$.  As illustrated in Figure \ref{fig:genplant}, this system describes the four transfer matrices from the disturbance and control inputs $w$ and $u$, respectively, to the controlled and measured outputs $y$ and $m$, respectively.  We make the (slightly modified) standard orthogonality assumptions that 
\begin{equation}
\begin{array}{rcl}
D_{12}\begin{bmatrix} C_1^\top & D_{12}^\top \end{bmatrix} &=&  \begin{bmatrix} 0 & \rho_u I \end{bmatrix}\\
 D_{21}^\top\begin{bmatrix} B_1 & D_{21} \end{bmatrix} &=&  \begin{bmatrix} 0 & \rho_w I \end{bmatrix}
\end{array}
\label{eq:ortho}
\end{equation}
 for some $\rho_u, \rho_w \geq 0$. \note{ At times we separate the state component of the open and closed loop responses from the components of these transfer matrices that measure control effort -- to that end, we define the \emph{state component} of an element $X \in \eltwoe$ to be the projection of $X$ onto the column space of $C_1$.}
 
 \edit{Letting $u(z) = K(z)m(z)$ for a causal linear controller $K\in\Rp$, the closed loop map from the disturbance $w$ to the measured output $m$ is given by the linear fractional transform $P_{11}-P_{12}K(I-P_{22}K)^{-1}P_{21}.$  A typical optimal control problem in this framework is then formulated as 
\begin{equation}
\begin{array}{rl}
\minimize{K\in\Rp} & \left\| P_{11}-P_{12}K(I-P_{22}K)^{-1}P_{21} \right\| \\
\text{s.t.} & K(I-P_{22}K)^{-1} \in \RHinf
\end{array}
\label{eq:OC}
\end{equation}
where $\|\cdot\|$ is a suitable norm, and the constraint ensures internal stability of the closed loop system \cite{ZDG96}.  Notice however that the optimal control problem \eqref{eq:OC} is non-convex as stated.}

\edit{
In order to reduce the technical overhead required, our discussion henceforth focusses on problems in which the generalized plant \eqref{eq:genplant} is open-loop stable, i.e. $|\lambda_{\max}(A)|<1$. In \edit{Remark \ref{rem:unstable} at the end of this subsection, we discuss how to extend our approach to unstable generalized plants \eqref{eq:genplant} through the use of recently developed structure preserving Youla-Kucera parameterizations built around \emph{arbitrary coprime factorizations}, which are always available \cite{SM12,MMRY12,LD14}.}
}
%It is also convenient to introduce finite horizon variants of these various operators.  Restricted to a finite horizon $n$, causal linear operators are isomorphic to block-lower triangular matrices.  We denote this subspace by $\T:= {\Rp^{\leq n}}$.

\edit{When the open-loop plant is stable, a standard and general approach to solving the optimal control problem \eqref{eq:OC} is to convert it into a \emph{model matching problem} through the \emph{Youla} change of variables $U:= K(I-P_{22}K)^{-1}$; the optimal controller $K$ can then be recovered via $K = (I+UP_{22})^{-1}U$.  The resulting convex optimization problem is then given by
\begin{equation}
\begin{array}{rl}
\minimize{U\in\RHinf} & \left\| P_{11}-P_{12}UP_{21} \right\|, \\
\end{array}
\label{eq:MM}
\end{equation}
which is precisely of the form of the linear inverse problem \eqref{eq:trad_opt} if we take $Y:= P_{11}$, $\Cl= P_{12}\otimes P_{21}$ (where we define $\left(P_{12}\otimes P_{21}\right)(U) := P_{12} U P_{21}$) and $\cost{U; Y,\Cl} := \left\| Y- \Cl(U)\right\|$.
}


%\note{Letting $u(z) = K(z)m(z)$ for a causal linear controller $K$, a general optimal control problem with cost function  \[\cost{X; P_{11}, P_{12}\otimes P_{21}}=\mu\left(P_{11} -  P_{12}XP_{21}\right),\] for some performance metric $\mu$, can then be written as 
%\begin{equation}
%\begin{array}{rl}
%\minimize{K\in\Rp} & \cost{K(I-P_{22}K)^{-1}; P_{11}, P_{12}\otimes P_{21}} \\
%\text{s.t.} &K(I-P_{22}K)^{-1} \in \RHinf
%\end{array}
%\label{eq:gen_opt}
%\end{equation}
% where the objective function corresponds to the size of the closed loop response of the disturbance input $w$ to the controlled output $y$ \cite{ZDG96} as measured by the performance metric $\mu$.  }

%When the additional distributed constraint that $K\in\s$ is not present, 
%\note{When the cost function $\cost{\cdot}$ is convex, a standard and general approach to solving the optimal control problem \eqref{eq:gen_opt} is to convert it into a \emph{model matching problem} through the \emph{Youla} change of variables $U:= K(I-P_{22}K)^{-1}$; the optimal controller $K$ can then be recovered via $K = (I+UP_{22})^{-1}U$.  The resulting optimization problem is then precisely of the form of the linear inverse problem \eqref{eq:trad_opt}, and is given by
%\begin{equation}
%\begin{array}{rl}
%\minimize{U\in\RHinf} & \cost{U; P_{11}, P_{12}\otimes P_{21}}.
%\end{array}
%\label{eq:cen_mm}
%\end{equation}}

%where $ \cost{U; P_{11}, P_{12}\otimes P_{21}} :=  \cost{P_{11}- P_{12}UP_{21}}$.}
%which is precisely of the form of the linear inverse problem \eqref{eq:trad_opt} with $Y := P_{11}$ and $\Cl(U) := P_{12}UP_{21}$.

We also often want to impose a \emph{distributed constraint}  on the controller $K$ by requiring $K$ to lie in some subspace $\s$, which specifies information exchange constraints between the sensors and actuators of the controller.  It is known that a necessary and sufficient condition for such a distributed constraint to be invariant under the Youla change of variables is that it be \emph{quadratically invariant} with respect to $P_{22}$ \cite{RL06,RCL10,LL11_QI}.

\begin{defn}[Quadratic Invariance]
A subspace $\s$ is \emph{quadratically invariant} (QI) with respect to $P_{22}$ if $KP_{22}K \in \s \ \forall K \in \s$.
\label{def:QI}
\end{defn}

In particular, when a subspace $\s$ is QI with respect to $P_{22}$, we have that $K \in \s$ if and only if $K(I-P_{22}K)^{-1} \in \s$, allowing us to convert the general optimal control problem \eqref{eq:trad_opt} with the additional constraint that $K\in\s$ to the following convex optimization problem

\begin{equation}
\begin{array}{rl}
\minimize{U\in\RHinf} & \cost{U; Y, \Cl}\\
\text{s.t.} & U \in \s.
\end{array}
\label{eq:gen_mm}
\end{equation}
\note{
%where $\cost{U; P_{11}, P_{12}\otimes P_{21}}$ is as defined for the centralized model matching problem \eqref{eq:cen_mm}. 
This optimization problem is again precisely of the form of the linear inverse problem \eqref{eq:trad_opt} save for the addition of the subspace constraint $U \in \s$.}
%By adding a RFD atomic norm penalty to optimization \eqref{eq:gen_mm}, we obtain a RFD optimization problem \eqref{eq:rfd_opt}.  


\edit{This framework is fairly general in that it allows for a unified treatment of all structured optimal control problems in which the linear optimal structured controller can be computed via convex optimization \cite{RL06,LL11_QI}.  These include state and output feedback problems in either centralized or QI distributed settings.  \edit{Further, when the optimal control problem is centralized with respect to the $\Htwo$, $\Hinf$ or $\mathcal{L}_1$ metric, or is QI distributed with respect to a finite horizon $\Htwo$ control cost, the linear optimal control is also globally optimal \cite{ZDG96,HC72,DahlehL1,LL11_QI}.}}

\edit{
\begin{rem}[Extension to Unstable Plants]
The above discussion extends to unstable plants through the use of an appropriate \emph{structure preserving} Youla-Kucera parameterization \edit{built around \emph{arbitrary coprime factorizations}}, which are always available.   See \cite{SM12,MMRY12,LD14} for examples of such parameterizations, and \cite{M_TCNS14} for an example of using such a parameterization in conjunction with a structure inducing penalty.
\label{rem:unstable}
\end{rem}}


%The rest of this section is organized as follows:  we first introduce the model matching framework in \S \ref{sec:model_match} and show how it maps to optimizations of the form \eqref{eq:trad_opt}.  In \S \ref{sec:RFDQI}, we show how \emph{quadratically invariant} distributed constraints can be accommodated, and more importantly that we can perform the architectural design task on the Youla parameter $U$, rather than the original controller.
%
\vspace{-2mm}

\subsection{Architecture Design through Structured Solutions}
\label{sec:RFDQI}

We seek a modification of the optimal controller synthesis procedure to design the controller's architecture.  We reiterate that by
the {architecture} of a controller, we mean the actuators, sensors, and communication links between them.  In particular, we view the controller $K$ as a map from all potential sensors to all potential actuators, using all potential communication links between these actuators and sensors.  The architectural design task is that of selecting which actuators, sensors and communication links need to be used to achieve a certain performance level.  This task is naturally viewed as one of finding a {structured approximation} of the optimal controller \eqref{eq:OC} that utilizes all of the available architectural choices.  

The components of the controller architecture being designed determine the type of structured approximation that we attempt to identify. In particular, each nonzero row of $K(z)$ corresponds to an actuator used by the controller, and likewise, each nonzero column corresponds to a sensor employed by the controller.  Further sparsity patterns present within rows/columns of the power series elements $K^{(t)}$ of $K(z)$ can be interpreted as information exchange constraints imposed by an underlying communication network between the sensors and actuators.  With these observations, it is clear that specific sparsity patterns in $K$ have direct interpretations in terms of the architectural components of the controller: nonzero rows correspond to actuators, nonzero columns correspond to sensors, and additional sparsity structure corresponds to communication constraints.   

\note{Although we seek seek to identify a suitably structured controller $K$, for the computational reasons described in \S\ref{sec:model_match} it is preferable to solve a problem in terms of the Youla parameter $U$ as this parameterization leads to the convex optimization problem \eqref{eq:gen_mm}.  %We therefore describe a modification to the model matching problems \eqref{eq:cen_mm} and \eqref{eq:gen_mm}, rather than the equivalent optimal control problem \eqref{eq:gen_opt}.  
Therefore, in the following definition RFD problems are defined as a regularized version of the model matching problem \eqref{eq:gen_mm} with a penalty function added to the objective to induce suitable structure, rather than as a modification of the controller synthesis problem \eqref{eq:OC}.   In the sequel, we justify that for architectural design problems of interest, the structure underlying the controller $K$ is equivalent to the structure underlying the Youla parameter $U$;   to that end, we show that in the case of actuator, sensor, and/or QI communication topology design,\footnote{\edit{We restrict ourselves to communications delays that satisfy the triangle inequality defined in \cite{RCL10}. This assumption implies that information exchanged between sensors and actuators is transmitted along shortest delay paths in the underlying communication graph.}} the structure of the Youla parameter $U$ corresponds to the structure of the controller $K$.}

%\todo{Although we're looking for structure in $K$, but for computational reasons as described in IIIA, we would like to be able to solve a problem in terms of $U$.  We describe a modification of the model matching problem rather than the equivalent optimal control problem...  As a result, in the following definition RFD problems are defined as a regularized version of \eqref{eq:gen_mm}, with a penalty function added to the objective to induce suitable structure.  In the sequel, we justify that for architectural design problems of interest, that structure in the controller $K$ is equivalent to structure of the Youla parameter $U$.  hence obtaining a structured solution in the youla parameter $U$ corresponds to a structured solution in the underlying controller $K$. }
%Our approach is to modify the model matching problem \eqref{eq:gen_mm} so that structure that has a direct interpretation in terms of the controller $K$'s architecture is induced in the Youla parameter $U$.

%Within this framework, we show that designing the controller architecture is equivalent to designing suitably {structured} Youla parameters $U$.
%
%In order to compute such a structured solution $U$, we modify the problem \eqref{eq:gen_mm} by augmenting it with a penalty function, or regularizer, to induce structure in the optimization problem's solution.

\begin{defn}
Let $U, \, Y\in\RHinf$, and $\Cl:\RHinf \to \RHinf$ be of compatible dimension.  The optimization
\begin{equation}
\begin{array}{rl}
\minimize{U\in \RHinf} & \cost{U; Y, \Cl}+2\lambda\Omega\left(U\right) \\
\text{s.t.} & U \in \s
\end{array}
\label{eq:rfd_opt}
\end{equation}
is called a \emph{RFD optimization problem} with cost function $\cost{\cdot;Y,\Cl}$ and penalty $\Omega\left(\cdot\right)$.
\end{defn}

\begin{rem}[Static or Dynamic]
With the exception of the centralized state-feedback setting, it is known that the optimal linear controller is dynamic \cite{ZDG96}, and therefore restricting our analysis to dynamic controllers is natural.  In the centralized setting (given the equivalence between static and dynamic state-feedback), once an appropriate actuation architecture\footnote{For a system to be centralized, there can be no communication constraints, and for it to be state-feedback, there can be no sensing constraints, leaving only actuation architecture design as a possible RFD task.} is identified, traditional methods can then be used to solve for a static state-feedback controller restricted to that architecture.  Further as we show in Section \ref{sec:recovery}, the dynamic controller synthesis approach is amenable to analysis that guarantees {optimal structure recovery}.
\end{rem}

We discuss natural costs $\cost{\cdot;Y,\Cl}$ and penalties $\Omega\left(\cdot\right)$ in Section \ref{sec:RFD_algos}, and we focus now on justifying why we can perform the structural design on the Youla parameter $U$ rather than the controller $K$. 


% which has a direct interpretation in terms of the resulting {architecture} of the control system.  In other words, we seek an ``architecturally sparse'' approximation of a hypothetical optimal controller that maximally utilizes the available architectural resources.  
%
%\todo{come back to this and see if it makes sense}



%In particular, when we solve a RFD optimization problem,  we obtain a structured Youla parameter $U$.  To this structured parameter $U$ we associate a subspace $\D$ (the manner in which we do this is made precise in the sequel).  We show that this subspace is QI under all relevant plants  $P_{22}$, thus ensuring $K \in \D$, i.e., that the architectural structure of $U$ corresponds to the architectural structure of $K$.




% we can guarantee that $K =  (I+UP_{22})^{-1}U \in \s\cap\D$ only if $\s\cap\D$ is QI under $P_{22}$.
%\todo{We really care about structure in $K$.  Fortunately, the structure in $K$ corresponding to sparse actuation, sensing and communication translates directly to the same structure in $U$ thanks to QI properties.  This sparsity structure can be viewed as a designed subspace $\D$.}

%Our ultimate goal will be to augment first step towards computationally tractable approaches for the design of controller architectures is to show that the architectural structure in the controller $K$ maps directly onto the structure of the Youla parameter $U$ under mild conditions.  

%\begin{itemize}
%\item \textbf{Actuation design}: $\Omega$ should penalize the number of nonzero rows of $U(z)$.
%\item \textbf{Sensing design}: $\Omega$ should penalize the number of nonzero columns of $U(z)$.
%\item \textbf{Communication design}: $\Omega$ should penalize specific sparsity patterns within the the impulse response of $U(z)$ that correspond to an added communication link.
%\item \textbf{Joint design}: $\Omega$ should penalize a weighted sum of the actuation, sensing, or communication penalties, depending on the subset of the architecture that is being co-designed.
%\end{itemize}
%
%
%
%\todo{When we talk about designing structured controllers, we desire structure in K.  Based on the preceding discussion, the cost function is only convex in the U parameterization.  Therefore we need to ensure that any structured solution $U$ to (6), which is in the $U$ domain, also carries through to the structure in the $K$ domain.}
%As the structural co-design task is performed on the Youla parameter $U$, care must be taken to ensure that the designed structure is preserved under the change of variables \todo{reference K=bla}.  As elements in the subspace of block lower triangular matrices $\T$ form an algebra, we focus on ensuring that any additional structure imposed on $U$ is equivalently imposed on $K$ \todo{fix}.  
%\todo{structure corresponds to a subspace.  We get a structured controller, and corresponding to that structured controller is a subspace.  That subspace needs to be QI}.


\paragraph{Actuator Design}  \note{Recall that the actuators that a controller $K$ uses are identified by the nonzero rows of $K$: the actuator design problem therefore corresponds to finding a controller $K$ that achieves a good closed loop response and that is sparse row-wise.  We claim that this corresponds exactly to finding a row sparse solution $U$ to the RFD optimization problem \eqref{eq:rfd_opt}.  This is true because any subspace $\D$ that is defined solely in terms of row sparsity is QI with respect to any $P_{22}$.   In particular, it is easily verified that if $K \in \D$, then right multiplication leaves $\D$ invariant, i.e., $KX \in \D$ for all compatible $X$. It then follows from Definition \ref{def:QI} that $\D$ is QI with respect to any plant $P_{22}$.  We can extend this analysis to incorporate additional QI distributed constraints $\s$ by leveraging the results\footnote{In particular, since removing actuators does not change the communication delays between the remaining actuators and sensors, if the delay based conditions in \cite{RCL10}  hold when all actuators are present they also hold with any subset of them being present.} in \cite{RCL10}: in particular, if $\s$ is QI with respect to $P_{22}$, then so is $\D \cap \s$.}

\paragraph{Sensor Design }
\note{The sensors employed by a controller $K$ are identified by the nonzero columns of $K$, and we therefore seek controllers that are sparse column-wise.  This once again corresponds exactly to finding a column sparse solution $U$ to the RFD optimization problem \eqref{eq:rfd_opt}.  In particular any subspace $\D$ that is defined solely in terms of its column sparsity is QI with respect to any plant $P_{22}$: to see this note that left multiplication leaves such a subspace $\D$ invariant, and therefore $K \in \D$ implies that $XK\in\D$ for all compatible $X$.   We can incorporate additional QI distributed constraints $\s$ by once again leveraging the results in \cite{RCL10}.}

\paragraph{Joint Actuator and Sensor Design} \note{By virtue of the previous discussion joint actuator and sensor design corresponds to finding a controller $K$ that is simultaneously sparse row-wise and column-wise.  It follows immediately from the previous discussion that this corresponds exactly to finding a simultaneously row and column sparse solution $U$ to the RFD optimization problem \eqref{eq:rfd_opt}.  In particular, any subspace $\D$ defined solely in terms of row and column sparsity is QI with respect to any plant $P_{22}$, we can incorporate additional QI distributed constraints $\s$ by leveraging the results in \cite{RCL10}.}

\paragraph{Communication Design}
\note{In an analogous manner to the above, one can also associate subspaces to structures corresponding to suitable information exchange constraints that a distributed controller must satisfy.
Recall in particular that the information exchange constraints between the sensors and actuators of a controller $K$ are identified by the sparsity structure found within the nonzero rows and columns of $K$.  In \cite{M_TCNS14}, the first author showed that a specific type of sparsity structure in $K$ corresponds exactly to sensors and actuators exchanging information according to an underlying communication graph.
In particular, given a communication graph between sensors and actuators with adjacency matrix $\Gamma$, a distributed controller $K$ can be implemented using the graph defined by $\Gamma$ if the power series elements $K^{(t)}$ of the controller satisfy\footnote{We assume that $K$ is square to streamline presentation; cf. \cite{M_TCNS14} for the general case.} $\supp{K^{(t)}}\subseteq \supp{\Gamma^{t-1}}$.  The interpretation of the support nesting condition is that the delay from sensor $j$ to actuator $i$ is given by the length of the shortest path from node $j$ to node $i$ in the graph defined by $\Gamma$.  This support nesting condition thus defines the distributed subspace constraint $\s$ in which $K$ must lie -- based on the discussion in \S\ref{sec:model_match}, one can pose the distributed controller synthesis problem as a distributed model matching problem \eqref{eq:gen_mm} if and only if $\s$ is QI with respect to $P_{22}$.  In light of this, we consider the communication design task proposed in \cite{M_TCNS14}: given an initial graph with adjacency matrix $\Gamma_{\text{QI}}$ that induces a QI distributed subspace constraint $\s$, what minimal set of additional edges should be added to the graph to achieve a desired performance level.\footnote{It is shown in \cite{M_TCNS14} that under mild assumptions on the plant $P_{22}$, the propagation delays of $P_{22}$ can be used to define an adjacency matrix $\Gamma_{\text{QI}}$ that induces a distributed subspace constraint that is QI with respect to $P_{22}$.}  It is additionally shown in \cite{M_TCNS14} that any communication graph constructed in this manner results in a subspace constraint $\s$ that is QI with respect to $P_{22}$.  Therefore the structure imposed on the controller $K$ by an underlying QI communication graph corresponds exactly to the structure imposed on the Youla parameter $U$.
%Logical flow: 
%1) exchange of info happens on a graph
%2) We need this graph to be QI
%3) Assume we start with a QI graph and seek to augment it.
 }
 
%A simple way to ensure that the designed subspace $\D_{\text{dyn}}$ is QI with respect to the plant $P_{22}$ is to begin with a communication graph with adjacency matrix $\Gamma_{\text{QI}}$ that induces a subspace $\D_{\text{QI}}$ for which QI holds, and to then augment it with additional communication links so as to achieve a specific performance bound.  

\paragraph{Joint Communication, Actuator and/or Sensor Design}
%Designing communication constraints is a more involved task, the details of which are beyond the scope of this paper.  
\note{By virtue of the previous discussion and the results of \cite{RCL10}, combining QI communication design with actuator and/or sensor design still leads to the underlying structure of the controller $K$ corresponding to the underlying structure of the Youla parameter $U$.}

Thus for architecture design problems the RFD task can be performed via a model matching problem.

\begin{example}
Suppose that different RFD optimization problems are solved for a system with three possible actuators and three possible sensors, resulting in the various sparsity patterns in $U(z)$ shown on the far right of Figure \ref{fig:patterns}.  It is easily seen by inspection that the resulting sparsity patterns are QI. In particular Figures \ref{fig:patterns}a) through \ref{fig:patterns}c) correspond to centralized RFD optimization problems (this can be seen from the full matrices in the center of the LHS), and 2d) to a RFD optimization problem subject to lower triangular constraints, a special case of a nested information constraint\footnote{Nested information constraints are a well studied class of QI distributed constraints, cf. \cite{LL11, S13, SP10, TP14} for examples.}.

\begin{figure}[h!]
\centering
\includegraphics[width = .45\textwidth]{patterns}
\caption{Examples of QI sparsity patterns generated via a) actuator, b) sensor, and c) actuator/sensor RFD procedures without any distributed constraints, and d) actuator RFD subject to nested information constraints.}
\label{fig:patterns}
\end{figure}
\end{example}



==> rfd_proc.tex <==
We now introduce the convex optimization based RFD procedure for the co-design of an optimal controller and the architecture on which it is implemented.  The remaining computational challenge is the possibly infinite dimensional nature of the RFD optimization problem \eqref{eq:rfd_opt}.  To address this issue, we propose a two step procedure: first, a finite dimensional approximation of optimization problem \eqref{eq:rfd_opt} is solved to identify a potential controller architecture and its defining subspace constraint $\D$.  Once this architecture has been identified, a traditional (and possibly infinite dimensional) optimal control problem \eqref{eq:trad_opt} with Youla prameter restricted to lie in $\D\cap\s$ is then solved -- in particular, in many interesting settings the resulting optimal controller restricted to the designed architecture can then be computed exactly leveraging classical and recent results in the optimal controller synthesis literature \distcitations.

Formally, we begin by fixing a horizon $t$ and a controller order $v$.  We suggest initially choosing $t$ and $v$ to be small (i.e., 2 or 3), and then gradually increasing these parameters until a suitable controller architecture/control law pair is found.  Our motivations for this approach are twofold: (i) first, a smaller horizon $t$ and controller order $v$ lead to a smaller optimization problem that are computationally easier to solve; and (ii) as we show in the next section, smaller values of the horizon $t$ and the controller order $v$ can actually aid in the identification of optimal controller architectures.  

For a given performance metric $\cost{\cdot;Y,\Cl}$ and atomic norm penalty $\|\cdot\|_\Aa$, the two step RFD procedure consists of an architecture design step and an optimal control law design step:
\begin{enumerate}
\item \textbf{Architecture design:} Select the regularization weight $\lambda$ and solve the finite dimensional RFD optimization problem
\begin{equation}
\begin{array}{rl}
\minimize{} & \cost{U;Y^{\leq t}, \Cl^{\leq t,v}} + 2\lambda \Omega\left(U\right) \\
\text{s.t.} & U \in \RHinf^{\leq v} \cap \s.
\end{array}
\label{eq:rfd_opt_trunc1}
\end{equation}
The actuators, sensors and communication links defining the designed architecture are defined by the non-zero atoms that constitute the solution $\hat{U}$ to optimization problem \eqref{eq:rfd_opt_trunc1}.  These architectural components in turn define the corresponding subspace $\D$ in which a controller $K$ implemented on said architecture is constrained to lie.
\item \textbf{Optimal control law design:} Solve the infinite dimensional optimal control problem with Youla parameter additionally constrained to lie in the designed subspace $\D\cap \s$:
\begin{equation}
\begin{array}{rl}
\minimize{U \in \RHinf} & \cost{U;Y, \Cl} \\
\text{s.t.} & U \in \D \cap \s.
\end{array}
\label{eq:rfd_opt_full}
\end{equation}
If the resulting controller architecture and controller performance are acceptable, the RFD procedure terminates.  Otherwise, adjust $\lambda$ accordingly to vary the tradeoff between architectural complexity and closed loop performance.  If no suitable controller architecture/controller can be found, increase $t$ and $v$ and repeat the procedure.
\end{enumerate} 

\begin{rem}[Removing Bias] \note{The method of solving a regularized optimization problem to identify the architectural structure of a controller and then solving a standard model matching problem restricted to the identified architecture is analogous to a procedure that is commonly employed in structured inference.  In structured inference problems, a regularized problem is solved first to identify a subspace corresponding to the structure of an underlying model $U_*$.  Subsequently, a non-regularized optimization problem with solution restricted to that identified subspace is solved to obtain an unbiased estimator of the underlying model $U_*$.}
\end{rem}

\subsection{Simultaneous Actuator, Sensor and Communication Design Example}
\label{sec:large}
\input{large}

As this example demonstrates, the RFD procedure is very effective at identifying simple controller architectures that approximate the performance of a controller that maximally utilizes the available architectural resources. In the next section, we offer some theoretical justification for the success of our procedure by suitably interpreting the RFD optimization problem \eqref{eq:rfd_opt} in the context of approximation theory and by making connections to analogous problems in structured inference.
